Unified Reasoning about Robustness Properties of Symbolic-Heap Separation Logic

We introduce heap automata, a formalism for automatic reasoning about robustness properties of the symbolic heap fragment of separation logic with user-defined inductive predicates. Robustness properties, such as satisfiability, reachability, and acyclicity, are important for a wide range of reasoning tasks in automated program analysis and verification based on separation logic. Previously, such properties have appeared in many places in the separation logic literature, but have not been studied in a systematic manner. In this paper, we develop an algorithmic framework based on heap automata that allows us to derive asymptotically optimal decision procedures for a wide range of robustness properties in a uniform way. We implemented a protoype of our framework and obtained promising results for all of the aforementioned robustness properties. Further, we demonstrate the applicability of heap automata beyond robustness properties. We apply our algorithmic framework to the model checking and the entailment problem for symbolic-heap separation logic.

==> Makefile <==
.PHONY: default clean distclean


default: main.pdf main_report.pdf


main_report.pdf: *.tex biblio.bib
	pdflatex main_report

main.pdf: *.tex biblio.bib  
	pdflatex main

all:
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main && \
	pdflatex main_report && \
	bibtex main_report && \
	pdflatex main_report && \
	pdflatex main_report

spellcheck:
	for f in *.tex; do aspell check $$f; done
	



clean:
	rm -f *.aux *.log *.bbl *.blg *~ main.pdf *.out *.synctex.gz *.backup

distclean: clean
	rm -f main.pdf main_report.pdf


==> app-entailment-short.tex <==



\section{Proof of Lemma~\ref{thm:entailment:predicates}} \label{app:entailment:predicates}
The crux of the proof relies on the fact that each unfolding of $\PS_1\T{x}$ has exactly one canonical model up to isomorphism, i.e.,
\begin{align*}
 \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \SIZE{\MODELS{\rsha}} = 1 \tag{$\bigstar$}.
\end{align*}
%
This property is a direct consequence of two properties:
By Definition~\ref{def:entailment:determined}, $\rsha$ has at most one canonical model up to isomorphism, because $\SRD$ is determined.
Furthermore, each symbolic heap $\rsha \in \CALLSEM{\PS_1\T{x}}{\SRD}$ has at least one canonical model, because $\SRD$ is well--determined.
%
Then
%
  \begin{align*}
                       & \PS_1\T{x} \SAT{\SRD} \PS_2\T{x} \\
     ~\Leftrightarrow~ & \left[ \text{Definition of entailments} \right] \\
                       & \forall (\stack,\heap) \in \STATES \,.\, \stack,\heap \SAT{\SRD} \PS_1\T{x} ~\text{implies}~ \stack,\heap \SAT{\SRD} \PS_2\T{x} \\
     ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{thm:symbolic-heaps:fv-coincidence},~\STATES_{\T{x}} \DEFEQ \{ (\stack,\heap) \in \STATES ~|~ \DOM(\stack) = \T{x} \} \right] \\
                       & \forall (\stack,\heap) \in \STATES_{\T{x}} \,.\, \stack,\heap \SAT{\SRD} \PS_1\T{x} ~\text{implies}~ \stack,\heap \SAT{\SRD} \PS_2\T{x} \\
     ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{thm:symbolic-heaps:semantics} \right] \\
                       & \forall (\stack,\heap) \in \STATES_{\T{x}} . 
                         \exists \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} . \stack,\heap \SAT{\emptyset} \rsha 
                         \,\text{implies}\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} . \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ A~\rightarrow~B \equiv \neg A \vee B \right] \\
                       & \forall (\stack,\heap) \in \STATES_{\T{x}} . 
                         \neg \left( \exists \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} . \stack,\heap \SAT{\emptyset} \rsha \right) 
                       \,\text{or}\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} . \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \neg \exists x . A \equiv \forall x . \neg A \right] \\
                       & \forall (\stack,\heap) \in \STATES_{\T{x}} \,.\, 
                         \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \stack,\heap \not \SAT{\emptyset} \rsha 
                       ~\text{or}~ \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \forall x \forall y . A \equiv \forall y \forall x . A \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \forall (\stack,\heap) \in \STATES_{\T{x}} \,.\, 
                       \stack,\heap \not \SAT{\emptyset} \rsha ~\text{or}~ \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ A~\rightarrow~B \equiv \neg A \vee B \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} . \forall (\stack,\heap) \in \STATES_{\T{x}} . 
                       \stack,\heap \SAT{\emptyset} \rsha \,\text{implies}\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \forall x . A \rightarrow B \equiv \forall x \in A . B,~\text{Def.}~\ref{def:symbolic-heaps:models} \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \forall (\stack,\heap) \in \MODELS{\rsha} \,.\,
                         \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \SIZE{\MODELS{\rsha}} = 1~\text{by}~(\bigstar)~\text{and}~ \forall x \in \{y\} . A \equiv \exists x \in \{y\} . A  \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \exists (\stack,\heap) \in \MODELS{\rsha} \,.\,
                         \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \exists x \exists y . A \equiv \exists y \exists x . A  \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \exists (\stack,\heap) \in \MODELS{\rsha} \,.\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \SIZE{\MODELS{\rsha}} = 1~\text{by}~(\bigstar)~\text{and}~ \forall x \in \{y\} . A \equiv \exists x \in \{y\} . A  \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \forall (\stack,\heap) \in \MODELS{\rsha} \,.\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \forall x . A \rightarrow B \equiv \forall x \in A . B \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \forall (\stack,\heap) \in \STATES \,.\,  \\
                       & \qquad (\stack,\heap) \in \MODELS{\rsha} ~\text{implies}~ \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \text{Def.}~\ref{def:symbolic-heaps:models}:~(\stack,\heap) \in \MODELS{\rsha} ~\Leftrightarrow~ \DOM(\stack) = \T{x} ~\text{and}~ \stack,\heap \SAT{\emptyset} \rsha \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \forall (\stack,\heap) \in \STATES \,.\, 
                       \DOM(\stack) = \T{x} \\
& \qquad \text{and}~ \stack,\heap \SAT{\emptyset} \rsha ~\text{implies}~ \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \forall x . (A \wedge B) \rightarrow C \equiv \forall x \in A . B \rightarrow C \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \forall (\stack,\heap) \in \STATES_{\T{x}} \,.\, \\
                       & \qquad \stack,\heap \SAT{\emptyset} \rsha ~\text{implies}~ \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{thm:symbolic-heaps:fv-coincidence} \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} . \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} . \forall (\stack,\heap) \in \STATES . 
                       \stack,\heap \SAT{\emptyset} \rsha \,\text{implies}\, \stack,\heap \SAT{\emptyset} \rsh \\
     ~\Leftrightarrow~ & \left[ \text{Definition of entailments} \right] \\
                       & \forall \rsha \in \CALLSEM{\PS_1\T{x}}{\SRD} \,.\, \exists \rsh \in \CALLSEM{\PS_2\T{x}}{\SRD} \,.\, \rsha \SAT{\emptyset} \rsh. \qedhere
  \end{align*}
\qed




==> app-entailment-top-level-short.tex <==
\begin{comment}
%\subsection{Proof of Lemma~\ref{thm:entailment:free-vars}} \label{app:entailment:free-vars}
\section{Constructing Well-Determined SIDs} \label{app:entailment:free-vars}

%\paragraph{Lifting well-determinedness}
% The next step is to extend the applicability of Lemma~\ref{thm:entailment:pred-entail}
% to entailments between arbitrary symbolic heaps instead of single predicate calls only.
% %
% We first weaken our requirement that the left-hand side of an entailment is well-determined.
% %
% In fact, the establishment condition, which has been studied in Section~\ref{sec:zoo:establishment},
% suffices.

%
%This is shown by transforming a given established SID -- and analogously an established symbolic heap --
%first into a determined one and subsequently into a well-determined one.
%
In this section, we show that an established SID  -- and analogously an established symbolic heap --
can be automatically transformed into a well-determined one.
%
Intuitively, the main difference between an established symbolic heap $\sh$ and a determined one $\sha$
lies in their free variables:
%
Since each existentially quantified variable of $\sh$ is eventually allocated or equal to a free variable,
all variables apart from free variables are definitely unequal in $\sh$.
%
The same holds for $\sha$, but each free variable is additionally either definitely equal or definitely unequal
to any other variable of $\sha$ 
(cf. Section~\ref{sec:entailment}).
%(cf. Example~\ref{example:entailment:determined:explicit}).
%
Thus, the main idea to transform $\sh$ into a determined symbolic heap is to add explicit pure formulas
between each free variable and each other variable.
%

%

%
More formally, let
$\textrm{Cmp}(\T{y},\sh)$ be the set of all sets $\PURE{}$ consisting of exactly one pure formula
$x \sim y$ for each $x \in \VAR(\sh)$ and each $y \in \T{y}$,
where $\sh \in \SL{}{}$ and $\T{y}$ is some tuple of variables.
%
Then, the following construction is essential to transform symbolic heaps into determined ones.
%
\begin{definition} \label{def:entailment:det}
  Let $\sh = \SYMBOLICHEAP{}$ be an established symbolic heap with $\NOCALLS{\sh} = m$ .
  Moreover, let $\T{y}$ be a tuple of variables of length $k \geq 0$
  and $\Lambda \in \textrm{Cmp}(\T{y},\sh)$.
  %
  Then,
  \begin{align*}
    \textrm{det}(\sh,\T{y},\Lambda) ~\DEFEQ~ &
        \exists \BV{} ~.~ \SPATIAL{} \SEP \textrm{propagate}(\sh,\T{y}) : \PURE{} \cup \Lambda, \\
    \textrm{propagate}(\sh,\T{y}) ~\DEFEQ~ &
         (\PS_1,k)\FV{1}{}\T{y} \SEP \ldots (\PS_m,k)\FV{m}{}\T{y},
  \end{align*}
  where $(\PS_i^{\sh},\beta)$ is a predicate symbol of arity $\ARITY(\PS_i^{\sh}) + \beta$.
\end{definition}
%
\begin{example}
  Let $\sh$ denote the symbolic heap in the lower rule of predicate $\texttt{sll}$
  in Example~\ref{ex:srd}. Then $\textrm{det}(\sh,\FV{0}{\sh}, \emptyset)$ is given by
  \begin{align*}
    &\exists z ~.~
      \PT{\IFV{1}}{z} ~\SEP~ (\texttt{sll},2)\,z\,\IFV{2}\,\FV{0}{\sh} ~:~ \{ \IFV{1} \neq \IFV{2}\}.
      \qedhere
  \end{align*}
\end{example}
%
\begin{lemma} \label{thm:entailment:free-vars}
%
 Let $\SRD \in \SETSRD{}$ be established. Then one can construct an SID $\SRDALT$ with $\PRED(\SRD) \subseteq \PRED(\SRDALT)$ such that for each $\PS \in \PRED(\SRD)$, we have:
 %
 \begin{itemize}
  \item $\rsh$ is well-determined for each $\rsh \in \CALLSEM{\PS\FV{0}{}}{\SRDALT}$,
  \item $\rsh \ENTAIL{\SRD} \PS\FV{0}{}$ holds for each $\rsh \in \CALLSEM{\PS\FV{0}{}}{\SRDALT}$, and
  \item $\rsh \ENTAIL{\SRDALT} \PS\FV{0}{}$ holds for each $\rsh \in \CALLSEM{\PS\FV{0}{}}{\SRD}$. \qedhere
 \end{itemize}
%
\end{lemma}
%ppend
Here, the last two points ensure that models of predicate calls remain unchanged,
although their actual unfoldings might differ.
%
\begin{proof}
 We first construct a determined SID $\Omega$.
 For each $Y,Z \in \PRED(\SRD)$, we introduce a fresh predicate symbol
 $(Y,\ARITY(Z))$, i.e.
 %
 \begin{align*}
   & \PRED(\Omega) ~\DEFEQ~ \PRED(\SRD) ~\cup~ \{ (Y,\ARITY(Z))  ~|~ Y,Z \in \PRED(\SRD) \}.
 \end{align*}
 %
 Furthermore, for each arity $k$ of some predicate symbol in $\SRD$,
 $\Omega$ contains two kinds of rules:
 %
 First, there is a rule that propagates the free variables of a symbolic heap
 through all of its predicate calls while comparing it to every variable.
 Formally, we add a rule
 $\SRDRULE{\PS}{\textrm{det}(\sh,\FV{0}{\sh},\Lambda)}$
 for each $\SRDRULE{\PS}{\sh} \in \SRD$ and each $\Lambda \in \textrm{Cmp}(\FV{0}{\sh},\sh)$.
 %
 The second kind of rule continues the propagation and comparison of a selected tuple of variables initiated
 by the first rule.
 Formally, we add a rule
 $\SRDRULE{(\PS,k)}{\textrm{det}(\sh,\T{y},\Lambda)}$, 
 where $\T{y}$ is a tuple of $k$ fresh variables,
 for each $\SRDRULE{\PS}{\sh} \in \SRD$ and each $\Lambda \in \textrm{Cmp}(\T{y},\sh)$.
 %
 Then $\Omega$ is determined.
 %

 %
 To obtain a \emph{well}-determined SID,
 we apply the Refinement Theorem (Theorem~\ref{thm:compositional:refinement}) to $\Omega$
 and the heap automaton $\HASAT$ (cf. Theorem~\ref{thm:zoo:sat:property}) accepting all satisfiable reduced symbolic heaps.
 %
 This yields the desired SID $\SRDALT$ in which every unfolding of each predicate call is satisfiable and determined.
 %
% A formal proof of correctness is found in Appendix~\ref{app:entailment:free-vars}.
%
%\end{proof}
%
%Lemma~\ref{thm:entailment:free-vars}
%is also applicable to established symbolic heaps $\sh \in \SL{\SRD}{}$
% by first adding a rule $\SRDRULE{\PS}{\sh}$ to $\SRD$,
%where $\PS$ is a fresh predicate of arity $\NOFV{\sh}$.\todo{Perhaps
%  omit, becomes clear anyway through Algo 2?}
%
%Hence, it suffices to require the left-hand side of an entailment to be established
%in order to apply the decidability result
%presented in  Lemma~\ref{thm:entailment:pred-entail}.
%
%Moreover, it its decidable whether a symbolic heap is established due to Theorem~\ref{thm:zoo:establishment}.
%
%
%Hence, it suffices to require the left-hand side of an entailment to be established in order to apply the decidability result
%presented in  Lemma~\ref{thm:entailment:pred-entail}.
%
%Note that by Theorem~\ref{thm:zoo:establishment} it is decidable whether a symbolic heap is established.
%This property is decidable
%
% After this transformation, Lemma~\ref{thm:zoo:sat:property} can be applied to obtain an SID $\SRDALT$ in which each unfolding of each predicate call is satisfiable.
%
%Hence, to ensure decidability it suffices to require the left-hand side of an entailment to be established.
%
%
%\begin{proof}
% We briefly recall the construction from the paper.
%
% For each $Y,Z \in \PRED(\SRD)$, we introduce a fresh predicate symbol $Z_{Y}$ of arity $\ARITY(Y) + \ARITY(Z)$.
% Thus,
% %
% \begin{align*}
%   & \PRED(\SRDALT) ~\DEFEQ~ \PRED(\SRD) ~\cup~ \{ Z_{Y} ~|~ Y,Z \in \PRED(\SRD) \}.
% \end{align*}
% %
% Now, fix some $Y \in \PRED(\SRD)$ of arity $n$ and a tuple $\T{y}$ of $n$ fresh variables.
% %
% Moreover, given $\sh \in \SL{\SRD}{}$, let $\textrm{Cmp}(\T{y},\sh)$ denote the set of all
% sets of pure formulas $\Lambda$ consisting of exactly one pure formula
% $u \sim v$ for each $u \in \T{y}$ and each $v \in \VAR(\sh)$.
% %
% Further, let $\sh_{Y,\Lambda}$ be the symbolic heap obtained from $\sh$ by
% adding free variables $\T{y}$, substituting each predicate call $\PS\FV{i}{}$ by $\PS_{Y}\FV{i}{}\,\T{y}$,
% and adding $\Lambda$ to the set of pure formulas.
% %, and adding a pure formula $y = z$ or $y \neq z$ for each $y \in \T{y}$ and each $z \in \VAR(\sh)$.
% %
% With this auxiliary construction readily available, an SID $\Omega$ is constructed as follows.
% %
% For each $\PS \in \PRED(\SRD)$, we add a rule
% %
% \begin{align*}
%  \SRDRULE{\PS}{\exists \BV{} . \PS_{\PS}\FV{0}{}\,\BV{} \,:\, \{ \IFV{i} = \PROJ{\BV{}}{i} ~|~ 1 \leq i \leq \ARITY(\PS) \}}
% \end{align*}
% to $\Omega$.
% Moreover, for each $\SRDRULE{\PS}{\sh} \in \SRD$, $Y \in \PRED(\SRD)$, and $\Lambda \in \textrm{Cmp}(\T{y},\sh)$,
% a rule $\SRDRULE{\PS_{Y}}{\sh_{Y,\Lambda}}$ is added to $\Omega$.
% %
% Finally, we apply the Refinement Theorem (Theorem~\ref{thm:compositional:refinement}) to $\Omega$
% and the heap automaton $\HASAT$ (cf. Theorem~\ref{thm:zoo:sat:property}) accepting all satisfiable reduced symbolic heaps.
% % 
% This yields the desired SID $\SRDALT$ in which every unfolding of each predicate call is satisfiable.
 %
% First, we construct a determined SID $\Omega$.
% For each $Y,Z \in \PRED(\SRD)$, we introduce a fresh predicate symbol
% $(Y,\ARITY(Z))$, i.e.
% %
% \begin{align*}
%   & \PRED(\Omega) ~\DEFEQ~ \PRED(\SRD) ~\cup~ \{ (Y,\ARITY(Z))  ~|~ Y,Z \in \PRED(\SRD) \}.
% \end{align*}
% %
% Furthermore, for each arity $k$ of some predicate symbol in $\SRD$
% and some tuple $\T{y}$ of $k$ fresh variables,
% $\Omega$ contains two kinds of rules:
% % 
% First, there is a rule that propagates the free variables of a symbolic heap
% through all of its predicate calls while comparing it to every variable. 
% Formally, we add a rule
% $\SRDRULE{\PS}{\textrm{det}(\sh,\FV{0}{\sh},\Lambda)}$
% for each $\SRDRULE{\PS}{\sh} \in \SRD$ and each $\Lambda \in \textrm{Cmp}(\FV{0}{\sh},\sh)$.%
% \footnote{$\textrm{det}$ and $\textrm{Cmp}$ are introduced in Definition~\ref{def:entailment:det}.}
% %
% The second kind of rule continues the propagation and comparison of a selected tuple of variables initiated
% by the first rule.
% Formally, we add a rule
% $\SRDRULE{(\PS,k)}{\textrm{det}(\sh,\T{y},\Lambda)}$
% for each $\SRDRULE{\PS}{\sh} \in \SRD$ and each $\Lambda \in \textrm{Cmp}(\T{y},\sh)$.
% %
% Then $\Omega$ is determined.
% %
% 
% %
% To obtain a \emph{well}-determined SID, 
% we apply the Refinement Theorem (Theorem~\ref{thm:compositional:refinement}) to $\Omega$
% and the heap automaton $\HASAT$ (cf. Theorem~\ref{thm:zoo:sat:property}) accepting all satisfiable reduced symbolic heaps.
% %
% This yields the desired SID $\SRDALT$ in which every unfolding of each predicate call is satisfiable and determined.
 %

 %

 %
 A detailed proof of correctness is provided in~\TECHNICALREPORT.
\qed
%
\end{proof}

\end{comment}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Theorem~\ref{thm:entailment:top-level}} \label{app:entailment:top-level}
%
Recall from Definition~\ref{def:entailment:heapmodels} the set of all reduced symbolic heaps in $\SHCLASS$ (over the same free variables as $\sh$) entailing an unfolding of $\sh$:
 \begin{align*}
  & \USET{\sh}{\SRD}{\SRDCLASS} 
  \DEFEQ \{ \rsha \in \RSL{}{\SRDCLASS} ~|~ \NOFV{\rsha} = \NOFV{\sh} \,\text{and}\, \exists \rsh \in \CALLSEM{\sh}{\SRD} \,.\, \rsha \ENTAIL{\emptyset} \rsh \}
 \end{align*}
%
\begingroup
\def\thetheorem{\ref{thm:entailment:top-level}}
\begin{theorem}
 %
 Let $\alpha \in \N$ and $\SRD \in \SETSRD{\SRDCLASSFV{\alpha}}$ be established.
 %
 Moreover, for each predicate symbol $\PS \in \PRED(\SRD)$, 
 let there be a heap automaton over $\SHCENTAIL{\alpha}$ accepting 
 $\USET{\PS\T{x}}{\SRD}{\CENTAIL{\alpha}}$.
 % be $\CENTAIL{\alpha}$--compositional.
 %
 Then, for every well-determined symbolic heap $\sh \in \SL{\SRD}{}$, 
 there is a heap automaton over $\SHCENTAIL{\alpha}$ accepting
 $\USET{\sh}{\SRD}{\CENTAIL{\alpha}}$.
 %the set $\USET{\sh}{\SRD}{\CENTAIL{\alpha}}$ is $\CENTAIL{\alpha}$--compositional.
 %
\end{theorem}
\endgroup
%
  %
  The proof is by induction on the syntax of symbolic heaps.
  %
  Since each case requires the construction of a suitable heap automaton and a corresponding correctness proof, we split the proof across multiple lemmas, which are shown subsequently in the remainder of this section.
  %
  Furthermore, we make some preliminary remarks to reduce the technical effort.
  %

  %
  \begin{remark}
  \label{remark:entailment:top-level:track}
  We assume without loss of generality
  that every predicate call occurring in a symbolic heap $\sh \in \SHCENTAIL{\alpha}$
  is annotated with a state of the tracking automaton $\HATRACK$ introduced in
  Definition~\ref{def:zoo:track-automaton}.
  Thus, for every predicate call $\CALLN{i}{\sh}$, we assume the availability of 
  \begin{itemize}
    \item a set $A_i \subseteq \FV{i}{\sh}$ capturing all allocated variables in a (fixed)
          unfolding of $\CALLN{i}{\sh}$, and
    \item a finite set of pure formulas $\PURE{}_i$ over $\FV{i}{\sh}$ capturing all definite
          equalities and inequalities between variables in $\FV{i}{\sh}$. 
  \end{itemize}
  This assumption is an optimization that prevents us from applying 
  Lemma~\ref{thm:zoo:track:property} again and again to keep track
  of the aforementioned relationships between parameters of predicate calls.
  \end{remark}  
  %
  \begin{remark}
  \label{remark:entailment:top-level:alpha}
  Furthermore, by Definition~\ref{def:entailment:centail}, 
  every predicate call has at most $\alpha$ parameters.
  %that are not obtained
  %from applying Lemma~\ref{thm:entailment:free-vars} to obtain a well-determined SID.
  %
  %Note that, by Definition~\ref{def:entailment:centail}, the number of parameters, 
  %which are not obtained from constructing a determined SID 
  %as explained in the proof of Lemma~\ref{thm:entailment:free-vars}, 
  %are bounded by some constant $\alpha$.
  %
  However, the number of free variables of the symbolic heap itself, 
  i.e. the formula at the root of an unfolding tree, 
  is not necessarily bounded by $\alpha$.
  %
  To avoid additional case distinctions in correctness proofs, we present
  constructions where the number of free variables is bounded by $\alpha$ as well.
  %
  In each of our constructions,
  this corner case can be dealt with by adding one dedicated final state $q_{>\alpha}$
  such that $(\EMPTYSEQ,\rsh,q_{> \alpha}) \in \Delta$ if and only if
  the number of free variables $\NOFV{\rsh}$ is greater than $\alpha$
  and the property in question is satisfied by $\rsh$.
  %
  General symbolic heaps with more than $\alpha$ free variables are treated analogously.
  %
  Once the final state $q_{> \alpha}$ has been reached no further transition is possible.
  Thus, only symbolic heaps at the root of an unfolding tree may enter $q_{>\alpha}$.
  \end{remark}
%
%
  %
  The remainder of the proof is summarized as follows:
  %
  \begin{itemize}
   \item The base cases $\PT{x}{\T{y}}$ and $\EMP$ are shown in Section~\ref{sec:entailment:points-to} and Section~\ref{sec:entailment:emp}, respectively.
   %
   \item For predicate calls $\PS\FV{0}{}$,
         we already know by assumption that $\USET{\PS\T{x}}{\SRD}{\CENTAIL{\alpha}}$
         is accepted by a heap automaton over $\SHCENTAIL{\alpha}$.
         %Thus, for each predicate symbol $\PS \in \PRED(\SRD)$,
         %there exists a heap automaton $\HASH{\PS\FV{0}{}}$ over $\CENTAIL{\alpha}$ accepting $\USET{\PS\T{x}}{\SRD}{\CENTAIL{\alpha}}$.
   %
   \item Section~\ref{sec:entailment:sepcon} shows that $\USET{\sh \SEP \sha}{\SRD}{\CENTAIL{\alpha}}$ is 
         accepted by a heap automaton over $\SHCENTAIL{\alpha}$  
         %$\CENTAIL{\alpha}$--compositional 
         if $\sh,\sha$ are defined over the same set of free variables.
         This is sufficient, because we do not require that these variables actually occur in both symbolic heaps.
   %
   \item Section~\ref{sec:entailment:pure} shows that $\USET{\sh : \Pi}{\SRD}{\CENTAIL{\alpha}}$ is 
         accepted by a heap automaton over $\SHCENTAIL{\alpha}$,
        % $\CENTAIL{\alpha}$--compositional, 
         where $\Pi$ is a finite set of pure formulas over the free variables of $\sh$.
   %
   \item Section~\ref{sec:entailment:existential} shows that $\USET{\exists z ~.~ \sh}{\SRD}{\CENTAIL{\alpha}}$ is 
         accepted by a heap automaton over $\SHCENTAIL{\alpha}$,
         %$\CENTAIL{\alpha}$--compositional, 
         where $z$ is a single variable.
         Repeated application then completes the proof.
  \end{itemize}
  %
  Hence, for each symbolic heap $\sh \in \SL{\SRD}{\CENTAIL{\alpha}}$, a corresponding heap automaton over $\SHCENTAIL{\alpha}$ accepting $\USET{\sh}{\SRD}{\CENTAIL{\alpha}}$ can be constructed.
  
  %
  For detailed correctness proofs of all lemmas in these sections, we refer to \TECHNICALREPORT.
  %
  %
\qed
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{The Points-to Assertion} \label{sec:entailment:points-to}
%
Let $\T{u} \in U_n = \{1, \ldots,\alpha\} \times \{0,1, \ldots,\alpha\}^{n-1}$ for some fixed natural number $n \geq 1$.
%
Moreover, we associate the points-to assertion
%
\begin{align*}
 \rsha_{\T{u}} ~\DEFEQ~ \PT{\PROJ{\FV{0}{}}{\PROJ{\T{u}}{1}}}{
    \PROJ{\FV{0}{}}{\PROJ{\T{u}}{2}} \ldots \PROJ{\FV{0}{}}{\PROJ{\T{u}}{n}}
 }
\end{align*}
%
with each tuple $\T{u} \in U_n$.\footnote{Recall that $\PROJ{\FV{0}{}}{0} = \NIL$.}
%
Then a heap automaton $\HASH{\rsha_{\T{v}}} = (Q,\SHCENTAIL{\alpha},\Delta,F)$ that accepts
$\USET{\rsha_{\T{v}}}{\SRD}{\CENTAIL{\alpha}}$ for some fixed tuple $\T{v} \in U_n$ is constructed as follows:
%
\begin{align*}
  Q ~\DEFEQ~ \{ \rsha_{\T{u}} ~|~ \T{u} \in U_n \} \cup \{\EMP\}
  \qquad
  F ~\DEFEQ~ \{ \rsha_{\T{v}} \}
\end{align*}
Moreover, for $\sh \in \SL{}{\CENTAIL{\alpha}}$ with $\NOCALLS{\sh} = m$,
 the transition relation $\Delta$ is given by:
%
\begin{align*}
              & \MOVE{\HASH{\rsha_{\T{v}}}}{q_0}{\sh}{q_1 \ldots q_m}
 \quad\text{iff}\quad %\begin{cases}
%                   \bigwedge_{1 \leq i \leq m} q_i \neq \bot
%                   ~\text{and}~
                    \REDUCE{\sh, q_1 \ldots q_m} \ENTAIL{\emptyset} q_0
%                   , & q_0 \neq \bot \\
%                   q_0 = \bot & \text{otherwise},
%                \end{cases}
\end{align*}
%
where $\REDUCE{\sh, q_1 \ldots q_m} \DEFEQ \sh[\PS_1 / q_1 : \Pi_i, \ldots, \PS_m / q_m : \Pi_m]$ and each set $\Pi_i$ denotes the set of pure formulas obtained from the tracking automaton (see Definition~\ref{def:zoo:track}),
which is assumed to be readily available by 
 Remark~\ref{remark:entailment:top-level:track}. 
%Definition~\ref{def:entailment:centail}.
%
\begin{lemma} \label{thm:entailment:points-to:compositionality}
 $\HASH{\rsha_{\T{v}}}$ satisfies the compositionality property.
\end{lemma}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{The Empty Heap} \label{sec:entailment:emp}
%
A heap automaton $\HASH{\EMP}$ accepting $\USET{\EMP}{\SRD}{\CENTAIL{\alpha}}$ is constructed analogously to
$\HASH{\rsha_{\T{v}}}$, the heap automaton constructed for the points-to assertion in Section~\ref{sec:entailment:points-to}.
The only exception is that $F_{\HASH{\EMP}} \DEFEQ \{ \EMP \}$ is chosen as set of final states.\footnote{The set of points-to assertions $U_n$ in this construction can even be chosen to be the empty set.} Since the compositionality property for this automaton already has been shown in Lemma~\ref{thm:entailment:points-to:compositionality}, it suffices to show
that $\HASH{\EMP}$ accepts the correct language.
%
\begin{lemma}
  $L(\HASH{\EMP}) = \USET{\EMP}{\SRD}{\CENTAIL{\alpha}}$.
\end{lemma}
%
\subsection{The Separating Conjunction}  \label{sec:entailment:sepcon}
%
Some additional notation is needed.
%
First, we write $\sh \equiv \sha$ if two symbolic heaps $\sh,\sha$ are identical up to the ordering of spatial formulas.
%
Given symbolic heaps $\sh$,$\sha$ and some variable $x$, we define
%
\begin{align*}
  [x]_{\sh,\sha} ~\DEFEQ~
    \begin{cases}
      x & ~\text{if}~x \in \VAR(\sh) \cup \VAR(\sha) \\
      \EMPTYSEQ & ~\text{otherwise}.
    \end{cases}
\end{align*}
%
Moreover, given two tuples $\T{x}$,$\T{y}$ taken from a finite set of variables $\{z_1,\ldots,z_n\}$, let $\T{x} \uplus \T{y} \DEFEQ [z_1]_{\sh,\sha} \,.\, \ldots \,.\, [z_n]_{\sh,\sha}$.
%
%
Similar to splitting a heap $\heap = \heap_1 \uplus \heap_2$ into two heaps, we define an operation to split \emph{symbolic} \emph{heaps}.
%
\begin{definition} \label{def:entailment:uplus}
 %
 Let $\sh,\sha \in \SL{}{}$ with free variables $\FV{0}{\sh}$, $\FV{0}{\sha}$ and
 %
 \begin{align*}
   \Gamma^{\sh} ~=~ \PS_1\FV{1}{\sh} \SEP \ldots \SEP \PS_m\FV{m}{\sh}
   ~\text{and}~
   \Gamma^{\sha} ~=~ \PS_1\FV{1}{\sha} \SEP \ldots \SEP \PS_m\FV{m}{\sha}.
 \end{align*}
 %
 Moreover, let $\BV{\sh},\BV{\sha} \subseteq \{z_1,\ldots,z_n\}$ for some $n \in \N$ and for each $0 \leq i \leq m$, let $\FV{i}{\sh},\FV{i}{\sh} \subseteq \FV{i}{}$, where $\FV{i}{}$ is some finite set of variables.
 %
 Then $\sh \uplus \sha$ is defined as
 %
 \begin{align*}
   \sh \uplus \sha ~\DEFEQ~ & \exists (\BV{\sh} \uplus \BV{\sha}) ~.~ \SPATIAL{\sh} \SEP \SPATIAL{\sha} \SEP \Gamma : \PURE{\sh} \cup \PURE{\sha}, \text{where} \\
   %
   \Gamma ~\DEFEQ~ & \PS_1(\FV{1}{\sh} \uplus\FV{1}{\sha}) \SEP \ldots \SEP \PS_m(\FV{m}{\sh} \uplus\FV{m}{\sha})
 \end{align*}
 %
 with free variables $\FV{0}{\sh} \uplus \FV{0}{\sha}$.%
 %
 \footnote{Note that technically, the predicate symbols $\PS_i$ may have different arities for each of the aforementioned symbolic heaps due to different numbers of parameters. This can easily be fixed by renaming predicate symbols. However, we chose to ignore the arity here to improve readability.}
 %
 Otherwise, $\sh \uplus \sha$ is undefined.
 %
\end{definition}
%
Since inequalities between allocated variables of a symbolic heap $\sh$ are redundant, let $\KERNEL(\sh)$ denote the corresponding symbolic heap in which such inequalities are removed.
%
Formally, $\KERNEL(\sh)$ is given by:
%
\begin{align*}
 \SYMBOLICHEAP{\sh} \setminus \{ a \neq b ~|~ a,b \in \ALLOC{\sh} \cup \{\NIL\} \}.
\end{align*}
%
Note that $\KERNEL(\sh)$ is computable in polynomial time if $\sh$ is reduced or each predicate is attached with variable tracking information (see Definition~\ref{def:zoo:track-automaton}).

%

%
We are now in a position to deal with the separating conjunction of two symbolic heaps.
%
Let $\sha_1,\sha_2 \in \SL{}{\CENTAIL{\alpha}}$ with $\VAR(\sha_1) = \VAR(\sha_2) = \FV{0}{\sha_1} = \FV{0}{\sha_2}$.
%
Moreover, let $\HASH{\sha_1}$, $\HASH{\sha_2}$ be heap automata over $\SHCENTAIL{\alpha}$ accepting $\USET{\sha_1}{\SRD}{\CENTAIL{\alpha}}$ and $\USET{\sha_2}{\SRD}{\CENTAIL{\alpha}}$, respectively.
%
We construct a heap automaton $\HASH{\sha_1 \SEP \sha_2} = (Q,\SHCENTAIL{\alpha},\Delta,F)$ accepting $\USET{\sha_1 \SEP \sha_2}{\SRD}{\CENTAIL{\alpha}}$ as follows:
%
\begin{align*}
   Q ~\DEFEQ~ & 2^{\T{u}} \times Q_{\HASH{\sha_1}} \times 2^{\T{u}} \times Q_{\HASH{\sha_2}} \times 2^{\T{u}}
   %
   \\
   %
   F ~\DEFEQ~ & 2^{\T{u}} \times F_{\HASH{\sha_1}} \times 2^{\T{u}} \times F_{\HASH{\sha_2}} \times 2^{\T{u}},~
\end{align*}
%
where $\T{u}$ denotes a tuple of $\alpha$ variables.
%
The main idea of choosing this state space is that each state $(U,p,V,q,H)$ stores the current states $p,q$ of heap automata $\HASH{\sha_1}$ and $\HASH{\sha_2}$ running on two separated symbolic heaps that are obtained from splitting the originally given symbolic heap into two parts.
%
These splitted symbolic heaps require some synchronization information encoded in sets $U,V,K$.
%
More precisely, $U,V$ store which free variables of the original symbolic heap belong to the symbolic heap fed into $\HASH{\sha_1}$ and $\HASH{\sha_2}$, respectively.
%
Finally, $H$ stores which variables are \emph{allocated} in the symbolic heap fed into $\HASH{\sha_1}$.
%
Correspondingly, all other allocated variables must be allocated in the symbolic heap fed into $\HASH{\sha_2}$.
%
These sets are checked in the transition relation to ensure compositionality.
%
Formally, for $\sh \in \SL{}{\CENTAIL{\alpha}}$ with $\NOCALLS{\sh} = m$, the transition relation $\Delta$ is given by:
%
\begin{align*}
                & (U_1,p_1,V_1,q_1,H_1) \ldots (U_m,p_m,V_m,q_m,H_m) \\
                & \qquad \xrightarrow{\sh}_{\HASH{\sha_1 \SEP \sha_2}} (U_0,p_0,V_0,q_0,H_0) \\
                %
   ~\text{iff}~ & \exists \sha_p,\sha_q ~.~ \KERNEL(\sh) \equiv \sha_p \uplus \sha_q \\
                %
                & \quad \text{and}~ \MOVE{\HASH{\sha_1}}{p_0}{\sha_p}{p_1 \ldots p_m} ~\text{and}~ \MOVE{\HASH{\sha_2}}{q_0}{\sha_q}{q_1 \ldots q_m} \\
                %
                & \quad \text{and}~ \forall 0 \leq i \leq m \,.\, \forall 1 \leq j \leq \alpha ~.~ \\
                %
                & \qquad \quad~~ \left( \PROJ{\T{u}}{j} \in U_i ~\text{iff}~ \PROJ{\FV{i}{\sh}}{j} \in \FV{i}{\sha_p}  \right) \\
                %
                & \qquad \text{and}~ \left( \PROJ{\T{u}}{j} \in V_i ~\text{iff}~ \PROJ{\FV{i}{\sh}}{j} \in \FV{i}{\sha_q}  \right) \\
                %
                & \qquad \text{and}~ \left( \PROJ{\T{u}}{j} \in H_i ~\text{iff}~ \PROJ{\FV{i}{\sh}}{j} \in \ALLOC{\sha_p}  \right).
\end{align*}
%
\begin{lemma}
 $\HASH{\sha_1 \SEP \sha_2}$ satisfies the compositionality property.
\end{lemma}
%
%
\begin{lemma}
 $L(\HASH{\sha_1 \SEP \sha_2}) = \USET{\sha_1 \SEP \sha_2}{\SRD}{\CENTAIL{\alpha}}$.
\end{lemma}
%
%
\subsection{The Pure Formula}  \label{sec:entailment:pure}
%
Dealing with pure formulas is rather straightforward, because we already know how to track equalities and inequalities using the construction from Definition~\ref{def:zoo:track-automaton}.
%

%
Let $\shb \in \SL{}{\CENTAIL{\alpha}}$ be a symbolic heap such that %$\USET{\shb}{\SRD}{\CENTAIL{\alpha}}$  $\CENTAIL{\alpha}$--compositional, i.e., 
there exists a heap automaton $\HASH{\shb}$ over $\SHCENTAIL{\alpha}$ %, say $\HASH{\shb}$, 
accepting $\USET{\shb}{\SRD}{\CENTAIL{\alpha}}$.
%
Moreover, let $\PURE{}$ be some finite set of pure formulas over the set of free variables of $\shb$.
%
We construct a heap automaton $\HASH{\shb : \PURE{}} = (Q,\SHCENTAIL{\alpha},\Delta,F)$ accepting $\USET{\sha}{\SRD}{\CENTAIL{\alpha}}$, where $\sha \DEFEQ \SYMBOLICHEAP{\shb} \cup \PURE{}$, as follows:
%
\begin{align*}
 Q ~\DEFEQ~ Q_{\HASH{\shb}} \times \{0,1\} \qquad F ~\DEFEQ~ F_{\HASH{\shb}} \times \{1\}.
\end{align*}
%
Moreover, for $\sh \in \SL{}{\CENTAIL{\alpha}}$ with $\NOCALLS{\sh} = m$, the transition relation $\Delta$ is given by:
%
\begin{align*}
              & \MOVE{\HASH{\shb : \PURE{}}}{(p_0,q_0)}{\sh}{(p_1,q_1) \ldots (p_m,q_m)} \\
 ~\text{iff}~ & \MOVE{\HASH{\shb}}{p_0}{\sh}{p_1 \ldots p_m} ~\text{and}~
                \bigwedge_{0 \leq i \leq m} q_i = 1 ~\text{iff}~ \PURE{} \subseteq \PURE{}_i,
\end{align*}
where $\PURE{}_i$ is the set of pure formulas obtained from the tracking automaton (see Definition~\ref{def:zoo:track-automaton}) that is available by Remark~\ref{remark:entailment:top-level:track}. 
%Definition~\ref{def:entailment:centail}.
%
\begin{lemma}
 $\HASH{\shb : \PURE{}}$ satisfies the compositionality property.
\end{lemma}
%
\begin{lemma}
 $L(\HASH{\shb : \PURE{}}) = \USET{\sha}{\SRD}{\CENTAIL{\alpha}}$, where $\sha \DEFEQ \SYMBOLICHEAP{\shb} \cup \PURE{}$ and $\shb \in \SL{\SRD}{\CENTAIL{\alpha}}$.
\end{lemma}
%
%
\subsection{The Existential Quantification}  \label{sec:entailment:existential}
%
In order to deal with existential quantifiers, we exploit the following structural property.
%
\begin{lemma} \label{thm:entailment:existential:structural-auxiliary}
  %
  For $\SRD \in \SETSRD{}$, let $\rsh \in \RSL{}{\alpha}$ be a well--determined symbolic heap and $\sha \in \SL{\SRD}{\alpha}$.
  %
  Moreover, let $x \notin \VAR(\rsh)$ and $\FV{0}{\sha} = \FV{0}{\rsh} \cdot x$.
  %
  Then $\rsh \ENTAIL{\SRD} \exists x \,.\, \sha$ holds if and only if there exists $y \in \VAR(\rsh)$ such that
  %
  %\begin{align*} &
    $\exists \BV{\rsh} . \SPATIAL{\rsh} : \PURE{\rsh} \cup \{ x = y \} \ENTAIL{\SRD} \sha$.% \qedhere
  %\end{align*}
  %
\end{lemma}
%
Exploiting the previous lemma, the main idea is to nondeterministically guess some
variable $y$ of an unfolding $\rsh$ and verify that $\rsh : \{ x = y\}$ belongs
to $\USET{\sha}{\SRD}{\CENTAIL{\alpha}}$.
%
Since this construction increases the number of free variables, we remark that $y$ has to be chosen carefully such that a symbolic heap in $\SL{}{\alpha}$ is obtained.
%
In particular, if $y$ does not belong to the root node of an unfolding tree, the corresponding predicate must either have an arity smaller than $\alpha$, or $y$ is equal to some other free variable.
%
However, each $y$ occurring in the root node of an unfolding tree may be chosen.
%

%
%
Before we present a formal construction, we first define how a symbolic heap $\sh$ is modified in the following.
%
\begin{definition}
  Let $\T{x}$ be a tuple of variables with $\SIZE{\T{x}} = n$.
  %
  Moreover, let $1 \leq k \leq n+1$. Then, the tuple of variables in which a fresh variable $x$ is placed at position $k$ is given by:
  %
  \begin{align*}
     \T{x}\SQUEEZE{x}{k} ~\DEFEQ~ \PROJ{\T{x}}{1}\, \ldots \, \PROJ{\T{x}}{k-1} ~ x ~ \PROJ{\T{x}}{k+1} \, \ldots \, \PROJ{\T{x}}{n}.
  \end{align*}
  %
  Now, let $\sh$ be a symbolic heap with $\NOFV{\sh} = \beta < \alpha$.
  %
  Then, the symbolic heap $\sh\SQUEEZE{x}{k}$ is defined as $\sh$ except for the tuple of free variables being $\FV{0}{\sh}\SQUEEZE{x}{k}$.
  %
  Furthermore, for some $1 \leq i \leq \NOCALLS{\sh}$ and $1 \leq \ell \leq \SIZE{\FV{i}{\sh}} + 1$,
  the symbolic heap $\sh\SQUEEZE{x}{i,\ell}$ is defined as $\sh$ except for the tuple of parameters of the $i$-th predicate call being $\FV{i}{\sh\SQUEEZE{x}{i,\ell}} = \FV{i}{\sh}\SQUEEZE{x}{\ell}$.
  %
  Otherwise, $\sh\SQUEEZE{x}{k}$ as well as $\sh\SQUEEZE{x}{i,k}$ are undefined.
\end{definition}
%
Now, let $\HASH{\sha}$ be a heap automaton accepting $\USET{\sha}{\SRD}{\CENTAIL{\alpha}}$ and $\HATRACK$ be the tracking automaton introduced in Definition~\ref{def:zoo:track-automaton}.
%
We construct a heap automaton $\HASH{\exists z.\sha} = (Q,\SHCENTAIL{\alpha},\Delta,F)$ accepting $\USET{\exists x . \sha}{\SRD}{\CENTAIL{\alpha}}$, where $x$ is the $k$-th free variable of $\sha$, as follows:
%
\begin{align*}
   Q ~\DEFEQ~ Q_{\HASH{\sha}} \times \{0,1,\ldots,\alpha\} \times Q_{\HATRACK} %\textnormal{Pure}(\FV{0}{} \cup \{y\})
   \qquad
   F ~\DEFEQ~ F_{\HASH{\sha}} \times \{k\} \times Q_{\HATRACK} %\textnormal{Pure}(\FV{0}{} \cup \{y\}).
\end{align*}
%
Moreover, for $\sh \in \SL{}{\CENTAIL{\alpha}}$ with $\NOCALLS{\sh} = m$, the transition relation $\Delta$ is given by:
%
\begin{align*}
                       & \MOVE{\HASH{\exists z. \sha}}{(p_0,q_0,r_0)}{\sh}{(p_1,q_1,r_m) \ldots (p_m,q_m,r_m)} \\
  \quad\text{iff}\quad &
                         \MOVE{\HASH{\sha}}{p_0}{\shb}{p_1 \ldots p_m}
                         ~\text{and}~
                         \MOVE{\HATRACK}{r_0}{\shb}{r_1 \ldots r_m}~,
\end{align*}
where $\shb$ adheres to one of the following cases:
%
\begin{enumerate}
 \item $q_0 = q_1 = \ldots = q_m = 0$ and $\shb = \sh$, or
 \item $q_0 = \ell > 0$ and there exists exactly one $1 \leq j \leq m$ such that $q_j = \ell' > 0$ and $\shb = (\sh\SQUEEZE{x}{\ell})\SQUEEZE{x}{j,\ell'}$, or
 \item $q_0 = \ell > 0$ and $\sum_{1 \leq i \leq m} q_i = 0$ and $\shb = (\sh\SQUEEZE{x}{\ell}) : \{ x = y \}$ for some $y \in \VAR(\sh)$.
\end{enumerate}
%
Here, $\sh : \{ y = x \}$ is a shortcut for the symbolic heap $\SYMBOLICHEAP{\sh} \cup \{ x = y \}$.
%
Moreover, the annotations of each predicate call $\CALLN{i}{\shb}$ are set to the sets contained in $r_i = (A_i,\Pi_i)$ instead of using existing annotations.
%
We remark that this construction is highly non-deterministic.
%
Furthermore, note that the automata rejects a symbolic heap if some $\shb$ does not belong to $\SL{}{\CENTAIL{\alpha}}$, because it is not a top-level formula and has more than $\alpha$ free variables.
%
\begin{lemma}
 $\HASH{\exists z.\sha}$ satisfies the compositionality property.
\end{lemma}
%
\begin{lemma}
 $L(\HASH{\exists z.\sha}) ~=~ \USET{\exists x . \sha}{\SRD}{\CENTAIL{\alpha}}$, where $x = \PROJ{\FV{0}{\sha}}{k}$ for some fixed position $k$.
\end{lemma}
%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> app-refinement-short.tex <==
\section{Proof of Theorem~\ref{thm:compositional:refinement}} \label{app:compositional:refinement}
%
The following lemma is essential to show that our construction of $\SRDALT$ is correct.
%
\begin{lemma} \label{thm:compositional:psi-correctness}
 Let $\SRD$, $\SRDALT$ and $\HA{A}$ be as in Theorem~\ref{thm:compositional:refinement}.
 %
 Then, for each $\PS \in \PRED(\SRD)$ and $q \in Q_{\HA{A}}$, we have
 %\begin{align*}
   $\rsh \in \CALLSEM{(\PS,q)\FV{0}{}}{\SRDALT} \quad\text{iff}\quad \rsh \in \CALLSEM{\PS\FV{0}{}}{\SRD} ~\text{and}~ \OMEGA{A}{q}{\rsh}$.
 %\end{align*}
\end{lemma}
%
\begin{proof}
  Let $\PS \in \PRED(\SRD)$ and $q \in Q_{\HA{A}}$.
  %
  By induction on the height $k$ of unfolding trees $t$, we show
    $t \in \UTREES{\SRDALT}{(\PS,q)\FV{0}{}}$
     iff there exists $t' \in \UTREES{\SRD}{\PS\FV{0}{}}$ such that $\UNFOLD{t'} = \UNFOLD{t}$ and
     $\OMEGA{A}{q}{\UNFOLD{t}}$.
  %
  Then
  %
  \begin{align*}
                      & \rsh \in \CALLSEM{(\PS,q)\FV{0}{}}{\SRDALT} \\
    ~\Leftrightarrow~ & \left[ \text{Definition}~\ref{def:symbolic-heaps:unfoldings} \right] \\
                      & \exists t \in \UTREES{\SRDALT}{(\PS,q)\FV{0}{}} ~.~ \UNFOLD{t} = \rsh \\
    ~\Leftrightarrow~ & \left[ \text{previously shown proposition} \right] \\
                      & \exists t' \in \UTREES{\SRD}{\PS\FV{0}{}} ~.~ \UNFOLD{t'} = \rsh ~\text{and}~ \OMEGA{A}{q}{\rsh} \\
    ~\Leftrightarrow~ & \left[ \text{Definition}~\ref{def:symbolic-heaps:unfoldings} \right] \\
                      & \rsh \in \CALLSEM{\PS\FV{0}{}}{\SRD} ~\text{and}~ \OMEGA{A}{q}{\rsh}
  \end{align*}
  which concludes the proof. \qed
  %
\end{proof}
%
We are now in a position to prove Theorem~\ref{thm:compositional:refinement}.
%
 It remains to show that for each $\PS \in \PRED(\SRD)$, we have $\CALLSEM{\PS\FV{0}{}}{\SRDALT} = \CALLSEM{P\FV{0}{}}{\SRD} \cap L(\HA{A})$.
 %
  By Lemma~\ref{thm:compositional:psi-correctness}, we know that for each $\PS \in \PRED(\SRD)$ and $q \in Q_{\HA{A}}$, we have
 \begin{align*}
   \rsh \in \CALLSEM{(\PS,q)\FV{0}{}}{\SRDALT} \quad\text{iff}\quad \rsh \in \CALLSEM{\PS\FV{0}{}}{\SRD} ~\text{and}~ \OMEGA{A}{q}{\rsh}. \tag{$\bigstar$}
 \end{align*}
 %
 %
 Then
 \begin{align*}
                     & \rsh \in \CALLSEM{\PS\FV{0}{}}{\SRDALT} \\
   ~\Leftrightarrow~ & \left[ \text{Definition}~\ref{def:symbolic-heaps:unfoldings} \right] \\
                     & \exists t \in \UTREES{\SRDALT}{\PS\FV{0}{}} ~.~ \UNFOLD{t} = \rsh \\
   ~\Leftrightarrow~ & \left[ \UNFOLD{t} = \PS\FV{0}{}[\PS\FV{0}{} / \UNFOLD{\SUBTREE{t}{1}}] = \UNFOLD{\SUBTREE{t}{1}} \right] \\
                     & \exists t \in \UTREES{\SRDALT}{\PS\FV{0}{}} ~.~ \UNFOLD{\SUBTREE{t}{1}} = \rsh \\
   ~\Leftrightarrow~ & \big[ \PS \SRDARROW (\PS,q) \in \SRDALT \Leftrightarrow q \in F_{\HA{A}},~ t(\EMPTYSEQ) = \PS\FV{0}{} 
                     ~\text{implies}~ \exists q \in F_{\HA{A}} . t(1) = (\PS,q)\FV{0}{} \big] \\
                     & \exists q \in F_{\HA{A}} . \exists t' \in \UTREES{\SRDALT}{(\PS,q)\FV{0}{}} ~.~ \UNFOLD{t'} = \rsh  \\
   ~\Leftrightarrow~ & \left[ \text{Definition}~\ref{def:symbolic-heaps:unfoldings} \right] \\
                     & \exists q \in F_{\HA{A}} ~.~ \rsh \in \CALLSEM{(\PS,q)\FV{0}{}}{\SRDALT} \\
   ~\Leftrightarrow~ & \left[ \text{applying}~(\bigstar) \right] \\
                     & \exists q \in F_{\HA{A}} ~.~ \rsh \in \CALLSEM{P\FV{0}{}}{\SRD} ~\text{and}~ \OMEGA{A}{q}{\rsh}. \\
   ~\Leftrightarrow~ & \left[ \rsh \in L(\HA{A}) \Leftrightarrow \exists q \in F_{\HA{A}} ~.~ \OMEGA{A}{q}{\rsh} \right] \\
                     & \rsh \in \CALLSEM{P\FV{0}{}}{\SRD} ~\text{and}~ \rsh \in L(\HA{A}) \\
   ~\Leftrightarrow~ & \left[ x \in A \wedge x \in B \Leftrightarrow x \in A \cap B \right] \\
                     & \rsh \in \CALLSEM{P\FV{0}{}}{\SRD} ~\cap~ \rsh \in L(\HA{A}). 
 \end{align*}
 \qed


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proof of Theorem~\ref{thm:refinement:boolean}} \label{app:refinement:boolean}
%
\begingroup
\def\thetheorem{\ref{thm:refinement:boolean}}
\begin{theorem}
  Let $\HA{A}$ and $\HA{B}$ be heap automata over $\SHCLASS$.
  %Let $H,K \subseteq \RSHCLASS$ be $\SRDCLASS$-compositional.
  Then there exists a heap automata $\HA{C}_1,\HA{C}_2,\HA{C}_3$ over $\SHCLASS$ with
  $L(\HA{C}_1) = L(\HA{A}) \cup L(\HA{B})$,
  $L(\HA{C}_2) = L(\HA{A}) \cap L(\HA{B})$, and
  $L(\HA{C}_3) = \RSHCLASS \setminus L(\HA{A})$, respectively.
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup
 %
\begin{proof}
 We split the proof across three lemmas that are proven subsequently.
 %
 Closure under union and intersection are shown in Lemma~\ref{thm:refinement:union} and Lemma~\ref{thm:refinement:intersection}, respectively.
 %
 Finally, closure under complement with respect to $\RSL{}{\SRDCLASS}$ is proven in Lemma~\ref{thm:refinement:complement}.
 %
 Correctness proofs of the provided constructions are found in~\TECHNICALREPORT.
 %
 \qed
 %
\end{proof}

%
\begin{lemma} \label{thm:refinement:union}
  Let $\HA{A},\HA{B}$ be heap automata over $\SHCLASS$. 
  Then there exists a heap automaton $\HA{C}$ over $\SHCLASS$ such that $L(\HA{C}) = L(\HA{A}) \cup L(\HA{B})$.
  %If $H$ and $K$ are $\SHCLASS$-compositional heap properties then $H \cup K$ is an $\SRDCLASS$--compositional heap property.
\end{lemma}
%
\begin{proof}
  %Let $\HA{A},\HA{B}$ be heap automata over $\SRDCLASS$ accepting $H$ and $K$.
  %
    We construct a heap automaton $\HA{C} = (Q,\SHCLASS,\Delta,F)$ accepting $L(\HA{A}) \cup L(\HA{B})$ %accepting $H \cup K$ 
  as follows:
  %
 \begin{align*}
   & Q ~\DEFEQ~ \left(Q_{\HA{A}} \cup \{\bot\}\right) \times \left(Q_{\HA{B}} \cup \{\bot\}\right) \\
   & F ~\DEFEQ~ F_{\HA{A}} \times \{\bot\} ~\cup~ \{\bot\} \times F_{\HA{B}} \\
   & \Delta ~:~ \MOVE{C}{(p_0,q_0)}{\sh}{(p_1,q_1)\ldots(p_m,q_m)} ~\Leftrightarrow~ \\
   & \qquad \qquad  \MOVE{A}{p_0}{\sh}{p_1 \ldots p_m} ~\text{and}~ p_2 = \bot ~\text{or} \\
   & \qquad \qquad  \MOVE{B}{q_0}{\sh}{q_1 \ldots q_m} ~\text{and}~ p_1 = \bot~,
 \end{align*}
 where $\sh \in \SL{}{\SRDCLASS}$ with $\NOCALLS{\sh} = m$.
 %
 Moreover, $\bot$ is assumed to be a fresh state.
 %
 \qed
 %
\end{proof}
%
\begin{lemma} \label{thm:refinement:intersection}
  Let $\HA{A},\HA{B}$ be heap automata over $\SHCLASS$. 
  Then there exists a heap automaton $\HA{C}$ over $\SHCLASS$ such that $L(\HA{C}) = L(\HA{A}) \cap L(\HA{B})$.
  %If $H$ and $K$ are $\SRDCLASS$-compositional heap properties then $H \cap K$ is an $\SRDCLASS$--compositional heap property.
\end{lemma}
%
\begin{proof}
  %Let $\HA{A},\HA{B}$ be heap automata over $\SRDCLASS$ accepting $H$ and $K$.
  %
    We construct a heap automaton $\HA{C} = (Q,\SHCLASS,\Delta,F)$ accepting $L(\HA{A}) \cap L(\HA{B})$ as follows:
  %
  \begin{align*}
   & Q ~\DEFEQ~ Q_{\HA{A}} \times Q_{\HA{B}} \qquad F ~\DEFEQ~ F_{\HA{A}} \times F_{\HA{B}} \\
   & \Delta ~:~ \MOVE{C}{(p_0,q_0)}{\sh}{(p_1,q_1)\ldots(p_m,q_m)} ~\Leftrightarrow~ \\
   & \qquad \MOVE{A}{p_0}{\sh}{p_1 \ldots p_m} ~\text{and}~ \MOVE{B}{q_0}{\sh}{q_1 \ldots q_m}~,
 \end{align*}
 where $\sh \in \SL{}{\SRDCLASS}$ with $\NOCALLS{\sh} = m$.
 %
 \qed
 %
\end{proof}
%
\begin{lemma} \label{thm:refinement:complement}
  Let $\HA{A}$ be a heap automaton over $\SHCLASS$.
  Then there exists a heap automaton $\HA{C}$ over $\SHCLASS$ such that 
  $L(\HA{C}) = \RSL{}{\SRDCLASS} \setminus L(\HA{A})$.
  %If $H$ is an $\SRDCLASS$-compositional heap property then $\RSL{}{\SRDCLASS} \setminus H$ is an $\SRDCLASS$--compositional heap property.
\end{lemma}
%
\begin{proof}
%
  %Let $\HA{A}$ be a heap automaton over $\SRDCLASS$ accepting $H$.
  %
  We construct a heap automaton $\HA{C} = (Q,\SHCLASS,\Delta,F)$ accepting
  $L(\HA{C}) = \RSL{}{\SRDCLASS} \setminus L(\HA{A})$ as follows:
%
 \begin{align*}
   & Q ~\DEFEQ~ 2^{Q_{\HA{A}}} \qquad F ~\DEFEQ~ \{ X \subseteq Q_{\HA{A}} ~|~ X \cap F_{\HA{A}} = \emptyset \} \\
   & \Delta ~:~ \MOVE{C}{X_0}{\sh}{X_1 \ldots X_m} ~\Leftrightarrow~ \\
   & \quad \forall q_0 \in X_0 . \forall 1 \leq i \leq m . \exists q_i \in X_i \,.\, \MOVE{A}{q_0}{\sh}{q_1 \ldots q_m} \\
   & \quad \text{and}~ \\
   & \quad \forall q_0 \notin X_0 . \forall 1 \leq i \leq m . \forall q_i \in X_i \,.\, \text{not}~ \MOVE{A}{q_0}{\sh}{q_1 \ldots q_m}~,
 \end{align*}
 where $\sh \in \SL{}{\SRDCLASS}$ with $\NOCALLS{\sh} = m$.
 %
 \qed
 %
\end{proof}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


==> app-symbolic-heaps-short.tex <==
\section{Supplementary Material} \label{app:supplement}

This section provides supplementary material, such as missing definitions.

\begin{definition}[Isomorphic states]
    Two states $(\stack_1,\heap_1), (\stack_2,\heap_2)$ are \emph{isomorphic} if and only if 
    there exist bijective functions $f : \DOM(\stack_1) \to \DOM(\stack_2)$
    $g : \DOM(\heap_1) \to \DOM(\heap_2)$ such that for all $\ell \in \DOM(\heap_1)$, we have
    $g(\heap_1(\ell)) = \heap_2(g(\ell))$, 
    where $g$ is lifted to tuples by componentwise application.
\end{definition}

\begin{lemma} \label{thm:symbolic-heaps:fv-coincidence}
 Let $\SRD \in \SETSRD{}$ and $\sh \in \SL{\SRD}{}$.
 %
 Moreover, let $(\stack,\heap) \in \STATES$.
 %
 Then
 $%\begin{align*}
    \stack,\heap \SAT{\SRD} \sh ~\text{iff}~ (\restr{\stack}{\FV{0}{\sh}}), \heap \SAT{\SRD} \sh,~
 $%\end{align*}
 where $\restr{\stack}{\FV{0}{\sh}}$ denotes the restriction of the domain of $\stack$ to the free variables of $\sh$.
\end{lemma}
%\endgroup
%
\begin{proof}
    By structural induction on the syntax of symbolic heaps $\sh$ (cf.~\TECHNICALREPORT for details).
  \qed
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> app-zoo-short.tex <==
%\begingroup
%\def\thelemma{\ref{thm:symbolic-heaps:fv-coincidence}}
%
%
%%%%% DONE %%%%%
\section{Proof of Lemma~\ref{thm:zoo:track:property}}
\label{app:zoo:track:property}
%
Note that some statements are broken down into separate lemmas which are
shown immediately afterwards.
%
\begingroup
\def\thelemma{\ref{thm:zoo:track:property}}
\begin{lemma}
 For all $\alpha \in \POSN$ and all sets
 $A \subseteq \FV{0}{}$, 
 $\PURE{} \in \textnormal{Pure}(\FV{0}{})$,
 %every set of pure formulas $\PURE{}$ over $\FV{0}{}$ with $\NOFV{} = \alpha$, and every set of variables $A \subseteq \FV{0}{}$,
there is a heap automaton over $\SHCLASSFV{\alpha}$ accepting
 $\TRACK(\alpha,A,\PURE{})$.
\end{lemma}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
  It suffices to show that the heap automaton $\HATRACK$ constructed in
  Definition~\ref{def:zoo:track-automaton} satisfies the compositionality
  property and accepts $\TRACK(\alpha,A,\PURE{})$.
  %
  We first show the latter, i.e., $L(\HATRACK) = \TRACK(\alpha,A,\PURE{})$.
  Let $\rsh \in \RSL{}{\SRDCLASSFV{\alpha}}$. Then
  %
  \begin{align*}
                       & \rsh \in L(\HATRACK) \\
     ~\Leftrightarrow~ & \left[ \text{Definition}~L(\HATRACK) \right] \\
                       & \exists (A',\Pi') \in F_{\HATRACK} ~.~ \OMEGA{\HATRACK}{(A',\Pi')}{\rsh} \\
     ~\Leftrightarrow~ & \left[ F_{\HATRACK} = \{(A,\Pi)\} \right] \\
                       & \OMEGA{\HATRACK}{(A,\Pi)}{\rsh} \\
     ~\Leftrightarrow~ & \left[ \text{Definition}~\Delta \right] \\
                       & \forall x,y \in \FV{0}{\rsh} ~.~
                           x \in A \leftrightarrow x \in \ALLOC{\SHRINK{\rsh,\EMPTYSEQ}} \\
                       & \qquad \text{and}~ (x \sim y) \in \Pi \leftrightarrow x \sim_{\SHRINK{\rsh,\EMPTYSEQ}} y \\
     ~\Leftrightarrow~ & \left[ \text{Definition}~\ref{def:zoo:track-automaton}:~\SHRINK{\rsh,\EMPTYSEQ} = \rsh  \right] \\
                       & \forall x,y \in \FV{0}{\rsh} ~.~
                           x \in A \leftrightarrow x \in \ALLOC{\rsh} ~\text{and}~ (x \sim y) \in \Pi \leftrightarrow x \sim_{\rsh} y \\
     ~\Leftrightarrow~ & \left[ \text{Definition}~\TRACK(\alpha,A,\Pi) \right] \\
                       & \rsh \in \TRACK(\alpha,A,\Pi).
  \end{align*}
  %
  The compositionality property of $\HATRACK$ is verified separately in
  Lemma~\ref{thm:zoo:track:compositional},
  which is proven in the remainder of this section.
  \qed
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma} \label{thm:zoo:track:compositional}
 Let $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m \geq 0$.
 %
 Moreover, for each $1 \leq i \leq m$, let $\rsh_i \in \RSL{}{\SRDCLASSFV{\alpha}}$ with $\SIZE{\FV{0}{\rsh_i}} = \SIZE{\FV{i}{\sh}}$.
 %
 Then, for $\rsh = \sh[\PS_1 / \rsh_1,\ldots \PS_m / \rsh_m]$, we have $\OMEGA{\HATRACK}{(A_0,\Pi_0)}{\rsh}$ if and only if there exist
 $(A_1,\Pi_1), \ldots, (A_m,\Pi_m) \in Q_{\HATRACK}$ such that
 %
  \begin{align*}
  \MOVE{\HATRACK}{(A_0,\Pi_0)}{\sh}{(A_1,\Pi_1) \ldots (A_m,\Pi_m)}
  \end{align*}
 %
 and, for each $1 \leq i \leq m$, we have $\OMEGA{\HATRACK}{(A_i,\Pi_i)}{\rsh_i}$.
\end{lemma}
%
\begin{proof}
  %
  Recall from Definition~\ref{def:zoo:track-automaton} that
  \begin{align*}
     \SHRINK{\sh,\T{q}} ~\DEFEQ~ &
        \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{q}[1]}, \ldots, \PS_m / \SSIGMA{\CALLN{m}{}}{\T{q}[m]}\right].
  \end{align*}
  %
  %
  Moreover, for each $1 \leq i \leq m$, let
  %
  \begin{align*}
    A_i ~\DEFEQ~ & \{ \PROJ{\FV{0}{}}{\ell} ~|~ \PROJ{\FV{0}{\rsh_i}}{\ell} \in \ALLOC{\rsh_i} \},~\text{and} \\
    \Pi_i ~\DEFEQ~ & \{ \PROJ{\FV{0}{}}{\ell} \sim \PROJ{\FV{0}{}}{k} ~|~ \PROJ{\FV{0}{\rsh_i}}{\ell} \MSIM{\rsh_i} \PROJ{\FV{0}{\rsh_i}}{k} \}.
  \end{align*}
  %
  Then
  %
  \begin{align*}
                      & \OMEGA{\HATRACK}{(A_0,\Pi_0)}{\rsh} \\
    ~\Leftrightarrow~ & \left[ \text{Definition of}~\Delta~\text{and}~ \SIZE{\CALLS{\rsh}} = 0  \right] \\
                      & \forall x,y \in \FV{0} ~.~ x \in A_0 ~\text{iff}~ x^{\sh} \in \ALLOC{\rsh} \\
                      & \qquad \text{and}~ x \sim y \in \Pi_0 ~\text{iff}~ x^{\sh} \MSIM{\rsh} y^{\sh} \\
    ~\Leftrightarrow~ & \left[ \text{choice of}~A_i~\text{and}~\Pi_i~\text{for each}~1 \leq i \leq m \right] \\
                      & \exists \T{q} = (A_1,\Pi_1) \ldots (A_m,\Pi_m) \in Q_{\HATRACK}^{m} ~.~ \forall x,y \in \FV{0} ~.~ \\
                      & \qquad x \in A_0 ~\text{iff}~ x^{\sh} \in \ALLOC{\rsh} \\
                      & \qquad \text{and}~ x \sim y \in \Pi_0 ~\text{iff}~ x^{\sh} \MSIM{\rsh} y^{\sh} \\
                      & \qquad \text{and}~ \forall 1 \leq i \leq m ~.~ \OMEGA{\HATRACK}{(A_i,\Pi_i)}{\rsh_i} \\
      ~\Leftrightarrow~ & \big[ \text{Lemma}~\ref{thm:zoo:track:congruence}~\text{(see below)} \big] \\
                      & \exists \T{q} = (A_1,\Pi_1) \ldots (A_m,\Pi_m) \in Q_{\HATRACK}^{m} ~.~ \forall x,y \in \FV{0} ~.~ \\
                      & \qquad x \in A_0 ~\text{iff}~ x^{\sh} \in \ALLOC{\SHRINK{\sh,\T{q}}} \\
                      & \qquad \text{and}~  x \sim y \in \Pi_0 ~\text{iff}~ x^{\sh} \MSIM{\SHRINK{\sh,\T{q}}} y^{\sh} \\
                      & \qquad \text{and}~ \forall 1 \leq i \leq m ~.~ \OMEGA{\HATRACK}{(A_i,\Pi_i)}{\rsh_i} \\
    ~\Leftrightarrow~ & \left[ \text{Definition of}~\Delta  \right] \\
                      & \exists \T{q} = (A_1,\Pi_1) \ldots (A_m,\Pi_m) \in Q_{\HATRACK}^{m} ~.~ \\
                      & \qquad \MOVE{A}{(A_0,\Pi_0)}{\sh}{(A_1,\Pi_1) \ldots (A_m,\Pi_m)} \\
                      & \qquad \text{and}~ \forall 1 \leq i \leq m ~.~ \OMEGA{\HATRACK}{(A_i,\Pi_i)}{\rsh_i}. 
  \end{align*}
  \qed
  %
\end{proof}
%
It remains to show that Lemma~\ref{thm:zoo:track:congruence}.
The crux of the proof of Lemma~\ref{thm:zoo:track:congruence} is the following observation.
%
\begin{lemma} \label{thm:zoo:track:congruence:auxiliary}
 Let $\sh = \exists \BV{} . \SPATIAL{} \SEP \CALLN{1}{} : \PURE{} \in \SL{}{\SRDCLASSFV{\alpha}}$.
 %
 Moreover, let $\rsh \in \RSL{}{}$ with $\SIZE{\FV{0}{\rsh}} = \SIZE{\FV{1}{\sh}}$, $A = \{ y \in \FV{0}{} ~|~ y^{\rsh} \in \ALLOC{\rsh} \}$ and $\Lambda = \{ x \sim y ~|~ x^{\rsh} \MSIM{\rsh} y^{\rsh} \}$.
 %
 Then, for each $x,y \in \VAR(\sh)$, we have
 %
 %
 \begin{align*}
    x \MSIM{\sh[\PS_1 / \rsh]} y \quad\text{iff}&\quad x \MSIM{\sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right]} y, \quad \text{and}~  \\
    x \in \ALLOC{\sh[\PS_1 / \rsh]} \quad\text{iff}&\quad x \in \ALLOC{\sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right]}~,
 \end{align*}
 %
 where $\SSIGMA{\CALLN{1}{}}{(A,\Lambda)}$ is defined in Section~\ref{sec:zoo} (above Definition~\ref{def:zoo:track-automaton}).
 %
\end{lemma}
%
Proving this lemma in turn relies on some auxiliary results, 
Lemma~\ref{thm:zoo:track-congruence-right} and Lemma~\ref{thm:zoo:track-congruence-left}, which are provided at the end of this section.
%
\begin{proof}
 %
 %
 \begin{align*}
                     & x \MSIM{\sh[\PS_1 / \rsh]} y \\
   ~\Leftrightarrow~ & \left[ \text{Definition of}~\MSIM{\sh[\PS_1 / \rsh]} \right] \\
                     & \forall (\stack,\heap) ~.~ \stack,\heap \SAT{\emptyset} \sh[\PS_1 / \rsh] ~\text{implies}~ \stack(x) \sim \stack(y) \\
   ~\Leftrightarrow~ & \left[ \text{logic} \right] \\
                     & \forall (\stack,\heap) ~.~ (\exists \heap' ~.~ \stack,\heap' \SAT{\emptyset} \sh[\PS_1 / \rsh]) ~\text{implies}~ \stack(x) \sim \stack(y) \\
   ~\Rightarrow~ & \left[ \text{Lemma}~\ref{thm:zoo:track:heap-existence} \right] \\
   %~\Leftrightarrow~ & \left[ \text{applying}~(\clubsuit) \right] \\
                     & \forall (\stack,\heap) ~.~ (\exists \heap' ~.~ \stack,\heap' \SAT{\emptyset} \sh[\PS_1 / \rsh]) ~\text{implies}~ \stack(x) \sim \stack(y) \\
                     & ~\text{and}~ \stack,\heap \SAT{\emptyset} \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right] \\
                     & \qquad ~\text{implies}~ (\exists \heap' ~.~ \stack,\heap' \SAT{\emptyset} \sh[\PS_1 / \rsh]) \\
       ~\Rightarrow~ & \left[ B \rightarrow C ~\wedge~ A \rightarrow B ~\text{implies}~ A \rightarrow C \right] \\
                     & \forall (\stack,\heap) ~.~ \stack,\heap \SAT{\emptyset} \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right] ~\text{implies}~ \stack(x) \sim \stack(y) \\
       ~\Leftrightarrow~ & \left[ \text{Definition of}~\MSIM{\sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right]} \right] \\
                     & x \MSIM{\sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right]} y.
 \end{align*}
 %
 Furthermore, we obtain
 %
 \begin{align*}
                     & x \in \ALLOC{\sh[\PS_1 / \rsh]} \\
   ~\Leftrightarrow~ & \left[ \text{Definition of}~\ALLOC{\sh[\PS_1 / \rsh]} \right] \\
                     & \forall (\stack,\heap) ~.~ \stack,\heap \SAT{\emptyset} \sh[\PS_1 / \rsh] ~\text{implies}~ \stack(x) \in \DOM(\heap) \\
   ~\Leftrightarrow~ & \left[ \text{logic} \right] \\
                     & \forall (\stack,\heap) ~.~ (\exists \heap' ~.~ \stack,\heap' \SAT{\emptyset} \sh[\PS_1 / \rsh] \\
                     & \qquad \text{and}~ \forall y \in \DOM(\stack) ~.~ \stack(y) \in \DOM(\heap) ~\text{iff}~ \stack(y) \in \DOM(\heap')) \\
                     & \quad \text{implies}~ \stack(x) \in \DOM(\heap) \\
   ~\Rightarrow~ & \left[ \text{Lemma}~\ref{thm:zoo:track:heap-existence} \right] \\
   %~\Leftrightarrow~ & \left[ \text{applying}~(\clubsuit) \right] \\
                     & \forall (\stack,\heap) ~.~ (\exists \heap' ~.~ \stack,\heap' \SAT{\emptyset} \sh[\PS_1 / \rsh] \\
                     & \qquad \text{and}~ \forall y \in \DOM(\stack) ~.~ \stack(y) \in \DOM(\heap) ~\text{iff}~ \stack(y) \in \DOM(\heap')) \\
                     & \qquad \quad \text{implies}~ \stack(x) \in \DOM(\heap) \\
                     & ~\text{and}~ \stack,\heap \SAT{\emptyset} \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right] \\
                     & \quad \text{implies}~ (\exists \heap' ~.~ \stack,\heap' \SAT{\emptyset} \sh[\PS_1 / \rsh] \\
                     & \qquad \text{and}~ \forall y \in \DOM(\stack) ~.~ \stack(y) \in \DOM(\heap) ~\text{iff}~ \stack(y) \in \DOM(\heap')) \\
       ~\Rightarrow~ & \left[ Y \rightarrow Z ~\wedge~ X \rightarrow Y ~\text{implies}~ X \rightarrow Z \right] \\
                     & \forall (\stack,\heap) ~.~ \stack,\heap \SAT{\emptyset} \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right] \\
                     & \qquad \text{implies}~ \stack(x) \in \DOM(\heap) \\
       ~\Leftrightarrow~ & \left[ \text{Definition of}~\ALLOC{\sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right]} \right] \\
                     & x \in \ALLOC{\sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right]}.
 \end{align*}
 %
 The proof of the converse direction is analogous, where the main difference is consists of using the property
 \begin{align*}
         & \stack,\heap ~\SAT{\emptyset}~ \sh[\PS_1 / \rsh] ~\text{implies}~\exists \heap' ~.~ \stack,\heap' \SAT{\emptyset}
           \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right] \\
         & \qquad ~\text{and}~ \forall y \in \DOM(\stack) ~.~
           \stack(y) \in \DOM(h) ~\text{iff}~ \stack(y) \in \DOM(\heap')
 \end{align*}
 instead of Lemma~\ref{thm:zoo:track:heap-existence}.
 This property is shown analogous to Lemma~\ref{thm:zoo:track:heap-existence} except that we apply Lemma~\ref{thm:zoo:track-congruence-left}
 instead of Lemma~\ref{thm:zoo:track-congruence-right}.
 %
 \qed
\end{proof}
%
\begin{lemma} \label{thm:zoo:track:congruence}
 %
 Let $\sh \in \SHCLASSFV{\alpha}$ with $\NOCALLS{\sh} = m \geq 0$.
 %
 For each $1 \leq i \leq m$, let $\rsh_i \in \RSHCLASSFV{\alpha}$ with $\NOFV{\rsh_i} = \SIZE{\FV{i}{\sh}}$, $A_i = \{ y \in \FV{0} ~|~ y^{\rsh_i} \in \ALLOC{\rsh_i} \}$ and $\PURE{}_i = \{ x \sim y ~|~ x^{\rsh_i} \MSIM{\rsh_i} y^{\rsh_i} \}$.
 %
 Moreover, let
 \begin{align*}
   \T{q} ~\DEFEQ~ & (A_1,\PURE{}_1) \ldots (A_m,\PURE{}_m), \\
   \rsh ~\DEFEQ~ & \sh\left[\PS_1 / \rsh_1, \ldots, \PS_m / \rsh_m\right],~\text{and} \\
   \SHRINK{\sh,\T{q}} ~\DEFEQ~ & \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{q}[1]}, \ldots, \PS_m / \SSIGMA{\CALLN{m}{}}{\T{q}[m]}\right].
 \end{align*}
 %
 Then, for each $x,y \in \VAR(\sh)$, we have
 \begin{align*}
   & x \in \ALLOC{\rsh} ~\text{iff}~ x \in \ALLOC{\SHRINK{\sh,\T{q}}}, ~\text{and} \\
   & x \MSIM{\rsh} y ~\text{iff}~ x \MSIM{\SHRINK{\sh,\T{q}}} y. \qedhere
 \end{align*}
 %
\end{lemma}
%
\begin{proof}
  We apply Lemma~\ref{thm:zoo:track:congruence:auxiliary} iteratively to
  %
  \begin{align*}
   \psi_0 ~=~ & \sh[\mathbf{P_1 / \rsh_1}, \PS_2 / \rsh_2, \ldots, \PS_m / \rsh_m] ~=~ \rsh \\
   \psi_1 ~=~ & \sh[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{q}[1]}, \mathbf{\PS_2 / \rsh_2}, \ldots, \PS_m / \rsh_m] \\
   \psi_2 ~=~ & \sh[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{q}[1]}, \PS_2 / \SSIGMA{\CALLN{2}{}}{\T{q}[2]}, \mathbf{\PS_3 / \rsh_3}, \ldots, \PS_m / \rsh_m] \\
              & \ldots \\
   \psi_i ~=~ & \sh[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{q}[1]}, \ldots, \PS_i / \SSIGMA{\CALLN{i}{}}{\T{q}[i]}, \\
              & \qquad  \mathbf{\PS_{i+1} / \rsh_{i+1}},\ldots \PS_m / \rsh_m] \big] \\
              & \ldots \\
  \psi_m ~=~ & \sh[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{q}[1]}, \ldots, \PS_m / \SSIGMA{\CALLN{m}{}}{\T{q}[m]}] = \SHRINK{\sh,\T{q}}.
  \end{align*}
  %
  Here, the replacement written in bold is the single predicate call to which Lemma~\ref{thm:zoo:track:congruence:auxiliary} is applied.
  %
  As a result, we obtain for each $0 \leq i,j \leq m$ and each pair of variables $x,y \in \VAR(\sh)$ that
  %
  \begin{align*}
    x \MSIM{\psi_i} y ~\text{iff}~ x \MSIM{\psi_j} y ~\text{and}~ x \in \ALLOC{\psi_i} ~\text{iff}~ x \in \ALLOC{\psi_j}.
  \end{align*}
  In particular, for $i = 0$ and $j = m$, this yields
  %
 \begin{align*}
   & x \in \ALLOC{\rsh} ~\text{iff}~ x \in \ALLOC{\SHRINK{\sh,\T{q}}}, ~\text{and} \\
   & x \MSIM{\rsh} y ~\text{iff}~ x \MSIM{\SHRINK{\sh,\T{q}}} y.
   %& x ~\MSIM{\rsh}~ y ~\text{iff}~  x ~\MSIM{\SHRINK{\sh,\T{q}}}~ y, ~\text{and} \\
   %& x \in \ALLOC{\rsh} ~\text{iff}~ x \in \ALLOC{\SHRINK{\sh,\T{q}}}. \qedhere
 \end{align*}
 \qed
  %
\end{proof}
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:track:heap-existence}
  Given the setting of Lemma~\ref{thm:zoo:track:congruence:auxiliary}, it holds that
  \begin{align*}
      & \stack,\heap \SAT{\emptyset} \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}\right] ~\text{implies} \\
    & \exists \heap' ~.~ \stack,\heap' \SAT{\emptyset} \sh[ \PS_1 / \rsh] ~\text{and}~ \forall y \in \DOM(\stack) ~.~ 
    \stack(y) \in \DOM(\heap) ~\text{iff} ~\stack(y) \in \DOM(\heap').
  \end{align*}
\end{lemma}
%
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:track-congruence-semantics}
 %
 Let $\rsh \in \RSL{}{}$, $A = \{ x \in \FV{0} ~|~ x^{\rsh} \in \ALLOC{\rsh} \}$ and $\Lambda = \{ x \sim y ~|~ x^{\rsh} \MSIM{\rsh} y^{\rsh} \}$.
 %
 Moreover, let $\SSIGMA{\CALLN{1}{}}{(A,\Lambda)}$ be defined as in Section~\ref{sec:zoo}.
 %
 Then, for each $(\stack,\heap) \in \STATES$ with $\DOM(s) = \FV{0}{\rsh}$, $\stack,\heap \SAT{\emptyset} \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}$ holds if and only if~\footnote{to be strict: $\heap = \{\ldots\}$ is a shortcut for $\DOM(\heap) = \{ \stack(x) ~|~ x \in A\}$, $\heap(\stack(x)) = \NIL$ for each $x \in A$}
 %
 %
 \begin{align*}
   & \heap = \{ \stack(x) \mapsto \NIL ~|~ x \in A \}
   ~\text{and}~ \bigwedge_{x \sim y \in \Lambda} \stack(x) \sim \stack(y)  \\
   & \text{and}~ \bigwedge_{x \in A, y \in (A \setminus \{x\}) \cup \{\NIL\}} \stack(x) \neq \stack(y).
 \end{align*}
 %
\end{lemma}
%
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:track-congruence-right}
 %
 Let $\rsh \in \RSL{}{}$, $A = \{ x \in \FV{0} ~|~ x^{\rsh} \in \ALLOC{\rsh} \}$ and $\Lambda = \{ x \sim y ~|~ x^{\rsh} \MSIM{\rsh} y^{\rsh} \}$.
 %
 Moreover, let $\SSIGMA{\CALLN{1}{}}{(A,\Lambda)}$ be defined as in Section~\ref{sec:zoo}.
 %
 Then, for each $(\stack,\heap) \in \STATES$ with $\DOM(s) = \FV{0}{\rsh}$, we have
 %
 \begin{align*}
   \stack,\heap \SAT{\emptyset} \SSIGMA{\CALLN{1}{}}{(A,\Lambda)} \quad\text{implies}\quad \exists h' ~.~ \stack,\heap' \SAT{\emptyset} \rsh.
 \end{align*}
 %
 Furthermore, for each $x \in \DOM(s)$, we have $\stack(x) \in \DOM(\heap)$ iff $\stack(x) \in \DOM(\heap')$.
 %
\end{lemma}
%
%\begin{proof}
% By structural induction on $\rsh$.
% \qed
    %\end{proof}
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:track-congruence-left}
 %
 Let $\rsh \in \RSL{}{}$, $A = \{ x \in \FV{0} ~|~ x^{\rsh} \in \ALLOC{\rsh} \}$ and $\Lambda = \{ x \sim y ~|~ x^{\rsh} \MSIM{\rsh} y^{\rsh} \}$.
 %
 Moreover, let $\SSIGMA{\CALLN{1}{}}{(A,\Lambda)}$ be defined as in Section~\ref{sec:zoo}.
 %
 Then, for each $(\stack,\heap) \in \STATES$ with $\DOM(s) = \FV{0}{\rsh}$, we have
 %
 \begin{align*}
   \stack,\heap \SAT{\emptyset} \rsh \quad\text{implies}\quad \exists h' ~.~ \stack,\heap' \SAT{\emptyset} \SSIGMA{\CALLN{1}{}}{(A,\Lambda)}.
 \end{align*}
 %
 Furthermore, for each $x \in \DOM(s)$, we have $\stack(x) \in \DOM(\heap)$ iff $\stack(x) \in \DOM(\heap')$.
 %
\end{lemma}
%
%%%%% DONE %%%%%
%
\section{Proof of Theorem~\ref{thm:zoo:sat:property}} \label{app:zoo:sat:property}

\begingroup
\def\thetheorem{\ref{thm:zoo:sat:property}}
\begin{theorem}
 For each $\alpha \in \POSN$, the set
 \begin{align*}
   \SATPROP(\alpha) ~\DEFEQ~ \{ \rsh \in \RSL{}{\SRDCLASSFV{\alpha}} ~|~ \rsh~\text{is satisfiable} \}
 \end{align*}
 of all satisfiable reduced symbolic heaps with at most $\alpha$ free variables can be accepted by a heap automaton over $\SHCLASSFV{\alpha}$.
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
    A heap automaton $\HASAT$ over $\SHCLASSFV{\alpha}$ accepting $\SATPROP(\alpha)$ is constructed as presented in Definition~\ref{def:zoo:track-automaton} except for the set of final states being set to
 %
    \[
  F_{\HASAT} ~\DEFEQ~ \{ (A,\Pi) ~|~ \NIL \neq \NIL \,\notin\, \Pi \}.
    \]
 %
 Since we already now that $\HATRACK$ and thus also $\HASAT$ satisfies the compositionality property (cf. Lemma~\ref{thm:zoo:track:compositional}), it suffices to show
 $L(\HASAT) = \SATPROP(\alpha)$.
 %
 Let $\rsh \in \RSL{}{\SRDCLASSFV{\alpha}}$. Then
 %
 \begin{align*}
                      & \rsh~\text{satisfiable} \\
    ~\Leftrightarrow~ & \left[ \text{Definition of satisfiability} \right] \\
                      & \exists (\stack,\heap) ~.~ \stack,\heap \SAT{\emptyset} \rsh \\
    ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{thm:symbolic-heaps:fv-coincidence} \right] \\
                      & \MODELS{\rsh} \neq \emptyset \\
    ~\Leftrightarrow~ & \big[ \big(\forall (\stack,\heap) \in \MODELS{\rsh} ~.~ \stack(\NIL) \neq \stack(\NIL)\big) 
                        ~\text{iff}~ \MODELS{\rsh} = \emptyset ] \\
                      & \exists \Pi ~.~ \forall x,y \in \FV{0}{\rsh} ~.~ \NIL \neq \NIL \notin \Pi \\
                      & \qquad \text{and}~ (x \sim y) \in \Pi \leftrightarrow \left( \forall (\stack,\heap) \in \MODELS{\rsh} ~.~ \stack(x^{\rsh}) \sim \stack(y^{\rsh}) \right) \\
    ~\Leftrightarrow~ & \left[ \text{Definition}~ x \MSIM{\rsh} y  \right] \\
                      & \exists \Pi ~.~ \forall x,y \in \FV{0}{\rsh} ~.~ \NIL \neq \NIL \notin \Pi 
                        ~\text{and}~ (x \sim y) \in \Pi \leftrightarrow x^{\rsh} \MSIM{\rsh} y^{\rsh} \\
    ~\Leftrightarrow~ & \left[ \text{Definition of}~F_{\HASAT} \right] \\
                      & \exists (A,\Pi) \in F_{\HASAT} ~.~ \forall x,y \in \FV{0}{\rsh} ~.~ x \in A \leftrightarrow x^{\rsh} \in \ALLOC{\rsh} \\
                        & \qquad \text{and}~ (x \sim y) \in \Pi \leftrightarrow x^{\rsh} \MSIM{\rsh} y^{\rsh} \\
    ~\Leftrightarrow~ & \left[ \text{Definition}~\ref{def:zoo:track-automaton}:~\SHRINK{\rsh,\EMPTYSEQ} = \rsh \right] \\
                      & \exists (A,\Pi) \in F_{\HASAT} ~.~ \forall x,y \in \FV{0}{\SHRINK{\rsh,\EMPTYSEQ}} ~.~ \\
                      & \qquad \qquad x \in A \leftrightarrow x^{\rsh} \in \ALLOC{\SHRINK{\rsh,\EMPTYSEQ}} \\
                      & \qquad \text{and}~ (x \sim y) \in \Pi \leftrightarrow x^{\rsh} \MSIM{\SHRINK{\rsh,\EMPTYSEQ}} y^{\rsh} \\
    ~\Leftrightarrow~ & \left[ \text{Definition}~\Delta_{\HASAT} \right] \\
                      & \exists (A,\Pi) \in F ~.~ \OMEGA{\HASAT}{(A,\Pi)}{\rsh} \\
    ~\Leftrightarrow~ & \left[ \text{Definition}~L(\HASAT) \right] \\
                      & \rsh \in L(\HASAT).
 \end{align*}
 Thus, $\rsh$ is satisfiable if and only if $\rsh \in L(\HASAT)$.
 \qed
 %
\end{proof}
%
%%%%% DONE %%%%%
\section{Satisfiability is in \CCLASS{NP}} \label{app:zoo:sat:np}
%
Brotherston et al.~\cite{brotherston2014decision} already showed that the satisfiability problem
is decidable in \CCLASS{NP} if the maximal number of free variables $\alpha$ is bounded.
%
In this section we briefly show that such an \CCLASS{NP}--decision procedure naturally emerged from our heap
automaton $\HASAT$ accepting $\SATPROP(\alpha)$ (see Theorem~\ref{thm:zoo:sat:property}).
%
\begin{lemma}
  \DPROBLEM{SL-SAT} is in \CCLASS{NP} if the maximal number $\alpha$ of free variables is bounded.
\end{lemma}
%
\begin{proof}
  Let $(\SRD,\sh) \in \DPROBLEM{SL-SAT}$ and $N = \SIZE{\SRD} + \SIZE{\sh}$.
  %~\footnote{We assume a reasonable function $\SIZE{.}$ determining the size of SRDs, formulas and unfolding trees, respectively.}
  %
  Moreover, let $n \leq N$ be the maximal number of predicate calls occurring in $\sh$ and any rule of $\SRD$.
  %
  Since $\alpha$ is a constant, the number of states of
  heap automaton $\HASAT$ (cf. the proof of Theorem~\ref{thm:zoo:sat:property})
  is a constant,
  %accepting \DPROBLEM{SL-SAT} is a constant,
  namely $k = 2^{2\alpha^2 + \alpha}$.
  %
  Now, let $\UTREES{\SRD}{\sh}^{\leq k}$ denote the set of all unfolding trees $t \in \UTREES{\SRD}{\sh}$ of height at most $k$.
  %
  Clearly, each of these trees is of size $\SIZE{t} \leq n^{k} \leq N^{k}$, i.e., polynomial in $N$.
  %
  Moreover, let $\omega: \DOM(t) \to Q_{\HASAT}$ be a function mapping each node of $t$ to a state of
  $\HASAT$. % heap automaton $\HAREACH$.
  %
  Again, $\omega$ is of size polynomial in $N$; as such $\SIZE{\omega} \leq k \cdot N^{k}$.
  %
  Let $\Omega_{t}$ denote the set of all of these functions $\omega$ for a given
  unfolding tree $t$ with $\omega(\EMPTYSEQ) \in F_{\HASAT}$.
  %
  Now, given an unfolding tree $t \in \UTREES{\SRD}{\sh}^{\leq k}$ and $\omega \in \Omega_{t}$, we can easily decide whether $\OMEGA{A}{\omega(\EMPTYSEQ)}{\UNFOLD{t}}$ holds:
  For each $u,u1,\ldots,un \in \DOM(t)$, $u(n+1) \notin \DOM(t)$, $n \geq 0$ it suffices to check whether $\MOVE{A}{\omega(u)}{t(u)}{\omega(u1) \ldots \omega(un)}$.
  %
  Since, by Remark~\ref{rem:closure}, 
  each of these checks can be performed in time polynomial in $N$,
  %$\BIGO{N^4}$ by 
  the whole procedure is feasible in polynomial time.
  % possible in $\BIGO{k \cdot N^{k+4}}$ and thus in polynomial time.

  %
  Then, our decision procedure for $\DPROBLEM{SL-SAT}$ answers yes on input $(\SRD,\sh)$ if and only if
  %
  \begin{align*}
    \exists t \in \UTREES{\SRD}{\sh}^{\leq k} ~.~ \forall \omega \in \Omega_{t} ~.~  \text{not}~ \OMEGA{A}{\omega(\EMPTYSEQ)}{\UNFOLD{t}}.
  \end{align*}
  %
  Since $t$ and $\omega$ are both of size polynomial in $N$, this procedure is in $\CCLASS{NP}$.
  %
  Regarding correctness, we first note that
  $\CALLSEM{\sh}{\SRD} \cap \SATPROP(\alpha) \neq \emptyset$ holds iff $\UNFOLD{t} \in \SATPROP(\alpha)$
  for some $t \in \UTREES{\SRD}{\sh}$.
  %
  Furthermore, by a standard pumping argument, it suffices to consider trees in $\UTREES{\SRD}{\sh}^{\leq k}$:
  If there exists a taller tree $t$ with $\UNFOLD{t} \in \SATPROP(\alpha)$ then there is some path of length greater $k$ in $t$ on which two nodes are assigned the same state by
  a function $\omega \in \Omega_{t}$ proving membership of $t$ in $\SATPROP(\alpha)$.
  Thus, this path can be shortened to obtain a tree of smaller height whose unfolding is satisfiable.
  %
  \qed
\end{proof}
%
%%%%% DONE %%%%%
\section{
Compositionality of $\HAEST$, $\HAGARBAGE$, $\HACYCLE$
}
\label{app:zoo:scheme:compositionality}
%
Some of our heap automata presented in Section~\ref{sec:zoo}
follow a common construction scheme.
%
In particular this holds for
%
\begin{itemize}
  \item $\HAEST$ (cf. Lemma~\ref{thm:zoo:establishment} and Appendix~\ref{app:zoo:establishment}),
  \item $\HAGARBAGE$ (cf. Lemma~\ref{thm:zoo:garbage:property} and Appendix~\ref{app:zoo:garbage:property}), and
  \item $\HACYCLE$ (cf. Lemma~\ref{thm:zoo:acyclicity:property} and Appendix~\ref{app:zoo:acyclicity:property}).
\end{itemize}
%
Intuitively, each of these automata evaluates a predicate
$\CHECK : \SL{}{\SRDCLASSFV{\alpha}} \times Q_{\HA{A}}^{*} \to \{0,1\}$
while running a heap automaton $\HA{A}$
-- which is either $\HATRACK$ (cf. Definition~\ref{def:zoo:track-automaton})
or $\HAREACH$ (cf. Lemma~\ref{thm:zoo:reachability:property})  --
in parallel to collect required knowledge about the relationships (equalities, allocation, reachability)
between free variables.
%

%
Due to these similarities, we prove the compositionality property for a general construction
scheme as described above.
%
%
More formally,
%
\begin{definition} \label{def:zoo:scheme-automaton}
  Let $\HA{A} \in \{ \HASAT, \HAREACH \}$
  be either the tracking automaton
  $\HATRACK$ (cf. Definition~\ref{def:zoo:track-automaton})
  or the reachability automaton
  $\HAREACH$ (cf. Lemma~\ref{thm:zoo:reachability:property}).
  %
  Moreover, let
  $F \subseteq Q_{\HA{A}} \times \{0,1\}$.
  %
  Further, let $\CHECK : \SL{}{\SRDCLASSFV{\alpha}} \times Q_{\HA{A}}^{\star} \to \{0,1\}$
  be a Boolean predicate such that for each
  $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m$
  $\rsh_1,\ldots,\rsh_m \in \RSL{}{\SRDCLASSFV{\alpha}}$,
  $\MOVE{A}{p_0}{\sh}{p_1 \ldots p_m}$, and $\OMEGA{A}{p_i}{\rsh_i}$,
  we have
  %
  \begin{align*}
   \CHECK(\sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m],\EMPTYSEQ) = 1
  \end{align*}
  if and only if such that
  \begin{align*}
    \CHECK(\sh, p_1 \ldots p_m) = \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1.
  \end{align*}
  %
  Then the heap automaton $\HASCHEME{\HA{A}}{\CHECK}{F}$ is given by
  \begin{align*}
   & \HASCHEME{\HA{A}}{\CHECK}{F} = (Q,\SHCLASSFV{\alpha},\Delta,F)~,\text{where} \\
   & Q ~\DEFEQ~ Q_{\HA{A}} \times \{0,1\} \\
   &  \Delta ~~:~~ \MOVE{B}{(p_0,q_0)}{\sh}{(p_1,q_1) \ldots (p_m,q_m)} \\
   & ~\text{iff}~ \MOVE{A}{p_0}{\sh}{p_1\ldots p_m} \\
   & \qquad ~\text{and}~ q_0 = \min \{q_1,\ldots,q_m,\CHECK(\sh,p_1 \ldots p_m)\}~,
  \end{align*}
  where $\NOCALLS{\sh} = m \geq 0$.
\end{definition}
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:scheme:compositionality}
  The heap automaton $\HA{B} = \HASCHEME{\HA{A}}{\CHECK}{F}$ satisfies the
  compositionality property.
\end{lemma}
  %
  %
%
%%%%% DONE %%%%%
%
\section{Proof of Theorem~\ref{thm:zoo:establishment}} \label{app:zoo:establishment}
%
%
\begingroup
\def\thetheorem{\ref{thm:zoo:establishment}}
\begin{theorem}
 %
 For each $\alpha \in \POSN$, the set
 %
 \begin{align*}
   \ESTPROP(\alpha) ~\DEFEQ~
   \{ \rsh \in \RSL{}{\SRDCLASSFV{\alpha}} ~|~ & \forall y \in \VAR(\rsh) ~.~ y \in \ALLOC{\rsh} 
                                                 ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y  \}
 \end{align*}
 %
 of all established reduced symbolic heaps having at most $\alpha$ free variables can be accepted by a heap automaton over $\SHCLASSFV{\alpha}$.
 %
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
%
We have to construct a heap automaton
$\HAEST$ over $\SHCLASSFV{\alpha}$ that satisfies the compositionality property
and accepts $\ESTPROP(\alpha)$.
%
In order to highlight the necessary proof obligations, the actual construction of $\HAEST$
and its correctness proof are splitted into several definitions and lemmas that are
provided afterwards.
%

%
The construction of $\HAEST$ was already sketched in the paper.
A fully formal construction of $\HAEST$ is found in Definition~\ref{def:zoo:establishment:automaton}.
%
It then remains to show the correctness of our construction of $\HAEST$:
%
\begin{itemize}
  \item Lemma~\ref{thm:zoo:establishment:language} establishes that $L(\HAEST) = \ESTPROP(\alpha)$.
  \item To prove the compositionality property, we show that $\HAEST$ is an instance of a more general
        construction scheme whose compositionality property is shown in
        Lemma~\ref{thm:zoo:scheme:compositionality}.
        In order to apply Lemma~\ref{thm:zoo:scheme:compositionality}, we have to show that
        \begin{align*}
                          & \CHECK(\sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m], \EMPTYSEQ) = 1 \\
             ~\text{iff}~ & \CHECK(\sh,p_1 \ldots p_m) = 1 ~\text{and}~ \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1.
         \end{align*}
         This is verified in Lemma~\ref{thm:zoo:establishment:compositionality}.
         By Lemma~\ref{thm:zoo:scheme:compositionality}, we then know that
         $\HAEST = \HASCHEME{\HATRACK}{\CHECK}{F}$ satisfies the compositionality property.
\end{itemize}
%
Putting both together, we obtain a heap automaton $\HAEST$ over $\SHCLASSFV{\alpha}$
that satisfies the compositionality property and accepts $\ESTPROP(\alpha)$.
Hence, $\ESTPROP(\alpha)$ is accepted by a heap automaton over $\SHCLASSFV{\alpha}$.
%
\qed
\end{proof}
%
%
The remainder of this section fills the gaps in the proof from above.
%
\begin{definition} \label{def:zoo:establishment:automaton}
$\HAEST = (Q,\SHCLASSFV{\alpha},\Delta,F)$ is given by
  %
  \begin{align*}
   & Q ~\DEFEQ~ Q_{\HATRACK} \times \{0,1\}, \qquad F ~\DEFEQ~ Q_{\HATRACK} \times \{1\}, \\
   &  \Delta ~~:~~ \MOVE{\HAEST}{(p_0,q_0)}{\sh}{(p_1,q_1) \ldots (p_m,q_m)} \\
   & ~\text{iff}~ \MOVE{\HATRACK}{p_0}{\sh}{p_1\ldots p_m} \\
   & \qquad \text{and}~ q_0 = \min \{q_1,\ldots,q_m,\CHECK(\sh,p_1 \ldots p_m)\}.
  \end{align*}
  Here, $\CHECK : \SHCLASSFV{\alpha} \times Q_{\HATRACK}^{*} \to \{0,1\}$ is a predicate given by
  \begin{align*}
   \CHECK(\sh,\T{p}) ~\DEFEQ~ \begin{cases}
                                   1 &, ~\text{if}~ \forall y \in \VAR(\sh) ~.~  y \in \ALLOC{\SHRINK{\sh,\T{p}}} \\
                                    & \qquad\text{or}~ \exists x \in \FV{0}{\sh} ~.~ x \MEQ{\SHRINK{\sh,\T{p}}} y \\
                                   0 &, ~\text{otherwise}~,
                                 \end{cases}
  \end{align*}
  where $\SHRINK{\sh,\T{p}}$ is the reduced symbolic heap obtained from the tracking property as in Definition~\ref{def:zoo:track-automaton}.
\end{definition}
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:establishment:language}
  $L(\HAEST) = \ESTPROP(\alpha)$.
\end{lemma}
%
\begin{lemma} \label{thm:zoo:establishment:compositionality}
  Let  $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m$
  and $\rsh_1,\ldots,\rsh_m \in \RSL{}{\SRDCLASSFV{\alpha}}$. Then
  %
  \begin{align*}
                   & \CHECK(\sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m], \EMPTYSEQ) = 1 \\
      ~\text{iff}~ & \CHECK(\sh,\T{p}) ~\text{and}~ \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1. 
  \end{align*}
  %
\end{lemma}
%
The proof of Lemma~\ref{thm:zoo:establishment:compositionality} relies
on a technical observation, which intuitively states that
%
equalities between variables belonging to different nodes of an unfolding tree have to be propagated through parameters.
%
Formally,
%
%\begin{lemma} \label{thm:zoo:establishment:equality-propagation}
\begin{lemma}[\TECHNICALREPORT] \label{obs:zoo:establishment:equality-propagation}
 Let  $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m$,  $\rsh_1,\ldots,\rsh_m \in \RSL{}{\SRDCLASSFV{\alpha}}$ and
 $\rsh = \sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m]$.
 %
 Moreover, for $1 \leq i \leq m$, let $x \in \VAR(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}])$ and $y \in \VAR(\rsh) \setminus \VAR(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}])$. Then
 $%\begin{align*}
    x \MEQ{\rsh} y \quad\text{iff}\quad \exists z \in \FV{i}{\sh} ~.~ x \MEQ{\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}]} z ~\text{and}~ z \MEQ{\rsh} y.
 $%\end{align*}
\end{lemma}
%
%
Note that $\NIL$ is always assumed to be a free variable and no other constants occur in our fragment of symbolic heaps.
Otherwise, the observation from above would be wrong.
%\end{lemma}
%

%
\begin{proof}[of Lemma~\ref{thm:zoo:establishment:compositionality}]
  %
  Let $\rsh = \sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m]$.
  %
  Recall that $\SHRINK{\rsh,\EMPTYSEQ}$ denotes the reduced symbolic heap
  introduced in Definition~\ref{def:zoo:track-automaton}.
  %
  Then:
  %
  \begin{align*}
     %
                       & \CHECK(\rsh,\EMPTYSEQ) = 1 \\
     ~\Leftrightarrow~ & \left[ \text{Definition of}~\CHECK,~\SHRINK{\rsh,\EMPTYSEQ} = \rsh \right] \\
                       & \forall y \in \VAR(\rsh) ~.~  y \in \ALLOC{\rsh} ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y \\
     ~\Leftrightarrow~ & \left[ \VAR(\rsh) = \VAR(\sh) \cup \bigcup_{1 \leq i \leq m} \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]) \right] \\
                       & \forall y \in \VAR(\sh) ~.~  y \in \ALLOC{\rsh} ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y \\
                       & \text{and}~ \forall 1 \leq i \leq m ~.~ \forall y \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right])  ~.~ y \in \ALLOC{\rsh} ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y \\
     ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{thm:zoo:track:congruence}~\text{applied to}~y \in \VAR(\sh) \text{and}~ x \in \VAR(\FV{0}{\rsh}) \right] \\
                       & \forall y \in \VAR(\sh) ~.~  y \in \ALLOC{\SHRINK{\sh,\T{p}}} 
                          ~\text{or}~ \exists x \in \FV{0}{\sh} ~.~ x \MEQ{\SHRINK{\sh,\T{p}}} y \\
                       & \text{and}~ \forall 1 \leq i \leq m ~.~ \forall y \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]) ~.~ 
                          y \in \ALLOC{\rsh} ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y \\
     ~\Leftrightarrow~ & \left[ \text{Definition of}~\CHECK \right] \\
                       & \CHECK(\SHRINK{\sh,\T{p}}) = 1 
                       ~\text{and}~ \forall 1 \leq i \leq m ~.~ \forall y \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]) ~.~ \\
                       & \qquad y \in \ALLOC{\rsh} ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y \\
     ~\Leftrightarrow~ & \big[ y \in \ALLOC{\rsh} ~\text{iff}~ y \in \ALLOC{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]} ~\text{or}~ \exists x \in \ALLOC{\rsh} ~.~ y \MEQ{\rsh} x \big] \\
                       & \CHECK(\SHRINK{\sh,\T{p}}) = 1 
                         ~\text{and}~ \forall 1 \leq i \leq m ~.~ \forall y \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]) ~.~ \\
                       & \qquad \left( y \in \ALLOC{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]} ~\text{or}~ \exists x \in \ALLOC{\rsh} ~.~ y \MEQ{\rsh} x\right)  
                       ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y \\
     ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{obs:zoo:establishment:equality-propagation} \right] \\
                       & \CHECK(\SHRINK{\sh,\T{p}}) = 1 ~\text{and}~ \forall 1 \leq i \leq m ~.~ \forall y \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]) ~.~ \\
                       & \qquad y \in \ALLOC{\rsh_i} ~\text{or}~ \exists z \in \FV{i}{\sh} . \exists x \in \ALLOC{\rsh} ~.~ y \MEQ{\rsh_i} z ~\text{and}~ z \MEQ{\rsh} x  \\
                       & \qquad \text{or}~ \exists x \in \FV{i}{\sh} . \exists z \in \FV{0}{\rsh} ~.~ y \MEQ{\rsh_i} x ~\text{and}~ x \MEQ{\rsh} z \\
     ~\Leftrightarrow~ & \big[ \FV{0}{\rsh_i}~\text{is substituted by}~\FV{i}{\sh} \in \VAR(\sh)~\text{in}~\rsh \\
                       & \qquad \text{which are all established due to $\CHECK(\SHRINK{\sh,\T{p}}) = 1$} \big] \\
                       & \CHECK(\SHRINK{\sh,\T{p}}) = 1 ~\text{and}~ \forall 1 \leq i \leq m ~.~ \forall y \in \VAR(\rsh_i) ~.~ \\
                       & \qquad y \in \ALLOC{\rsh_i} ~\text{or}~ \exists z \in \FV{0}{\rsh_i} ~.~ y \MEQ{\rsh_i} z \\
     ~\Leftrightarrow~ & \left[ \text{Definition of}~\CHECK \right] \\
                       & \CHECK(\SHRINK{\sh,\T{p}}) = 1 ~\text{and}~ \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1.
  \end{align*}
  \qed
  %
\end{proof}
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Lemma~\ref{thm:zoo:establishment:lower}} \label{app:zoo:establishment:lower}
%
\begingroup
\def\thelemma{\ref{thm:zoo:establishment:lower}}
\begin{lemma}
  \COMPLEMENT{SL-RSAT} is polynomial-time reducible to \DPROBLEM{SL-EST}.
  Hence, deciding $\DPROBLEM{SL-EST}$ is \CCLASS{ExpTime}--hard in general and \CCLASS{coNP}--hard if the maximal number of free variables is bounded.
\end{lemma}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}

%
 Let $(\SRD,\PS) \in \COMPLEMENT{SL-RSAT}$ be an instance of the complement of the reduced satisfiability problem.
 %
 Moreover, consider the instance $(\SRD,\sh)$ of the establishment problem, where
 %
 \begin{align*}
   \sh ~\DEFEQ~ \exists \T{z} z' ~.~ \PS\T{z} : \{ x = \NIL, z' \neq \NIL \}
 \end{align*}
 and $x$ is the single free variable (other than $\NIL$) of $\sh$.
 %
 Then
 %
 \begin{align*}
                      & \CALLSEM{\sh}{\SRD} \subseteq \ESTPROP(\alpha) \\
    ~\Leftrightarrow~ & \left[ A \subseteq B ~\text{iff}~ \forall x \in A . x \in B \right] \\
                      & \forall \rsh \in \CALLSEM{\sh}{\SRD} ~.~ \rsh \in \ESTPROP(\alpha) \\
    ~\Leftrightarrow~ & \left[ \text{Definition of}~\ESTPROP(\alpha) \right] \\
                      & \forall \rsh \in \CALLSEM{\sh}{\SRD} ~.~ \forall y \in \VAR(\rsh) ~.~ y \in \ALLOC{\rsh} ~\text{or}~ \exists x \in \FV{0}{\rsh} ~.~ y \MEQ{\rsh} x \\
    ~\Leftrightarrow~ & \left[ \SRD~\text{contains no points-to assertions} \right] \\
                      & \forall \rsh \in \CALLSEM{\sh}{\SRD} ~.~ \forall y \in \VAR(\rsh) ~.~ \exists x \in \FV{0}{\rsh} ~.~ y \MEQ{\rsh} x \\
    ~\Leftrightarrow~ & \left[ \PROJ{\FV{0}{\rsh}}{1} \MEQ{\rsh} \NIL \right] \\
                      & \forall \rsh \in \CALLSEM{\sh}{\SRD} ~.~ \forall y \in \VAR(\rsh) ~.~ y \MEQ{\rsh} \NIL \\
    ~\Leftrightarrow~ & \left[ z' \MNEQ{\rsh} \NIL \right] \\
                      & \forall \rsh \in \CALLSEM{\sh}{\SRD} ~.~ \NIL \MNEQ{\rsh} \NIL \\
    ~\Leftrightarrow~ & \left[ \NIL \MNEQ{\rsh} \NIL ~\text{iff}~ \rsh~\text{unsatisfiable} \right] \\
                      & \forall \rsh \in \CALLSEM{\sh}{\SRD} ~.~ \rsh~\text{is unsatisfiable} \\
    ~\Leftrightarrow~ & \left[ \forall x . \neg A \equiv \neg \exists x . A \right] \\
                      & \text{not}~\exists \rsh \in \CALLSEM{\sh}{\SRD} ~.~ \rsh~\text{if satisfiable} \\
    ~\Leftrightarrow~ & \left[ \text{Definition of satisfiability} \right] \\
                      & \sh~\text{is unsatisfiable}.
 \end{align*}
 %
 Then it remains to show that $\sh$ is unsatisfiable if and only if $\PS$ is unsatisfiable:
 \begin{align*}
                     & \exists (\stack,\heap) \in \STATES ~.~ (\stack,\heap) \SAT{\SRD} \sh \\
   ~\Leftrightarrow~ & \left[ \text{Applying}~(\spadesuit)~\text{see below} \right] \\
                     & \exists (\stack,\heap) \in \STATES ~.~ \exists \T{u} \in \VAL^{\SIZE{\T{z}}} ~.~ 
                        (\restr{\stack[\T{z} \mapsto \T{u}]}{\T{z}},\heap) \SAT{\SRD} \PS\T{z} \\
                     & \qquad \text{and}~ \stack(x) = \NIL ~\text{and}~ \stack(z') \neq \NIL \\
   ~\Leftrightarrow~ & \left[ \DOM(\restr{\stack[\T{z} \mapsto \T{z}]}{\T{z}}) = \T{z} \right] \\
                     & \exists (\stack,\heap) \in \STATES ~.~ (\stack,\heap) \SAT{\SRD} \PS\T{z}.
 \end{align*}
 %
 Here, the missing step marked with ($\spadesuit$) corresponds to the following property:
 \begin{align*}
                      & \stack,\heap \SAT{\SRD} \sh 
   ~\Leftrightarrow~  \exists \T{u} \in \VAL^{\SIZE{\T{z}}} ~.~ \tag{$\spadesuit$} \\
                      & (\restr{\stack[\T{z} \mapsto \T{u}]}{\T{z}}),\heap \SAT{\SRD} \PS\T{z}
                      ~\text{and}~ \stack(x) = \NIL ~\text{and}~ \stack(z') \neq \NIL.
 \end{align*}
 %
 To complete the proof, let $(\stack,\heap) \in \STATES$. Then:
 %
 \begin{align*}
                      & \stack,\heap \SAT{\SRD} \sh \\
    ~\Leftrightarrow~ & \left[ \text{Construction of}~\sh \right] \\
                      & \stack,\heap \SAT{\SRD}  \exists \T{z} z' ~.~ \PS\T{z} : \{ x = \NIL, z' \neq \NIL \} \\
    ~\Leftrightarrow~ & \left[ \text{SL semantics} \right] \\
                      & \exists \T{u} \in \VAL^{\SIZE{\T{z}}} . \exists v \in \VAL ~.~ \\
                      & \qquad \stack[\T{z} \mapsto \T{u}, z' \mapsto v],\heap \SAT{\SRD} \PS\T{z} \\
                      & \qquad \text{and}~ \stack[\T{z} \mapsto \T{u}, z' \mapsto v],\heap \SAT{\SRD} x = \NIL \\
                      & \qquad \text{and}~ \stack[\T{z} \mapsto \T{u}, z' \mapsto v],\heap \SAT{\SRD} z' \neq \NIL \\
    ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{thm:symbolic-heaps:fv-coincidence} \right] \\
                      & \exists \T{u} \in \VAL^{\SIZE{\T{z}}} . \exists v \in \VAL ~.~ \\
                      & \qquad (\restr{\stack[\T{z} \mapsto \T{u}, z' \mapsto v]}{\T{z}}),\heap \SAT{\SRD} \PS\T{z} \\
                      & \qquad \text{and}~ (\restr{\stack[\T{z} \mapsto \T{u}, z' \mapsto v]}{x}),\heap \SAT{\SRD} x = \NIL \\
                      & \qquad \text{and}~ (\restr{\stack[\T{z} \mapsto \T{u}, z' \mapsto v]}{z'}),\heap \SAT{\SRD} z' \neq \NIL \\
    ~\Leftrightarrow~ & \left[ \text{SL semantics} \right] \\
                      & \exists \T{u} \in \VAL^{\SIZE{\T{z}}} ~.~ (\restr{\stack[\T{z} \mapsto \T{u}]}{\T{z}}),\heap \SAT{\SRD} \PS\T{z} \\
                      & \qquad \text{and}~ \stack(x) = \NIL ~\text{and}~ \stack(z') \neq \NIL,
 \end{align*}
 which coincides with $(\spadesuit)$.
 \qed
 %
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Theorem~\ref{thm:zoo:reachability:property}}
\label{app:zoo:reachability:property}
%
%
\begingroup
\def\thetheorem{\ref{thm:zoo:reachability:property}}
\begin{theorem}
 %
  Let $\alpha \in \POSN$ and $R \subseteq \FV{0}{} \times \FV{0}{}$ be a binary relation over the variables $\FV{0}{}$ with $\SIZE{\FV{0}{}} = \alpha$.
  %
  Then the \emph{reachability} \emph{property} $\RPROP(\alpha,R)$, given by the set
  %
  \begin{align*}
    & \{ \rsh \in \RSHCLASSFV{\alpha} ~|~ \forall i,j ~.~ (\PROJ{\FV{0}{}}{i},\PROJ{\FV{0}{}}{j}) \in R  ~\text{iff}~ \REACH{\PROJ{\FV{0}{\rsh}}{i}}{\PROJ{\FV{0}{\rsh}}{j}}{\tau} \},
  \end{align*}
  %
  can be accepted by a heap automaton over $\SHCLASSFV{\alpha}$.
 %
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
We have to construct a heap automaton
$\HAREACH$ over $\SHCLASSFV{\alpha}$ that satisfies the compositionality property
and accepts $\RPROP(\alpha,R)$.
%
In order to highlight the necessary proof obligations, the actual construction of $\HAREACH$
and its correctness proof are splitted into several definitions and lemmas that are
provided afterwards.
%
%
The construction of $\HAREACH$ was already sketched in the paper.
%Recall from Definition~\ref{def:zoo:track-automaton} the construction of a
%heap automaton $\HATRACK$ accepting $\TRACK(\alpha,A,\Pi)$.
%%
%The crux of this construction is to replace each predicate by a reduced symbolic heap
%%
%\begin{align*}
%   \SSIGMA{\sh}{(B,\Lambda)}
%  % \rsha_{\rsh,B,\Lambda}
%   ~\DEFEQ~ \bigstar_{\PROJ{\FV{0}{}}{i} \in B} ~ \PT{\PROJ{\FV{0}{\sh}}{i}}{\NIL} ~:~ \Lambda.
%\end{align*}
%%
%which captures precisely the definite allocations, equalities and inequalities stored in its state space.
%%
%A heap automaton $\HAREACH$ accepting $\RPROP(\alpha,R)$ is constructed analogously except that $\HAREACH$ additionally stores a relation $S$ in its state space to remember which free variables are reachable from another.
%%
%Correspondingly, this additional information is encoded in a reduced symbolic heap
%%
%\begin{align*}
%   %\rsha_{\rsh,B,\Lambda,S}
%   \SSIGMA{\sh}{(B,\Lambda,S)}
%   ~\DEFEQ~ \exists z ~.~ \bigstar_{\PROJ{\FV{0}{}}{i} \in B} ~ \PT{\PROJ{\FV{0}{\sh}}{i}}{\T{v}_i} ~:~ \Lambda~,
%    %\cup \{ z \neq x ~|~ x \in \FV{0}{} \},
%\end{align*}
%%
%where $z$ is a fresh variable and
%$\PROJ{\T{v}_i}{j} \DEFEQ  \PROJ{\FV{0}{\sh}}{j}$ if $(i,j) \in S$ and
%$\PROJ{\T{v}_i}{j} \DEFEQ  z$, otherwise.
%
A formal construction is provided in Definition~\ref{def:zoo:reachability-automaton}.
%
It then remains to show the correctness of our construction of $\HAREACH$:
%
\begin{itemize}
  \item Lemma~\ref{thm:zoo:reachability:language} shows that $\HAREACH$ indeed
        accepts $\RPROP(\alpha,R)$, i.e., $L(\HAREACH) = \RPROP(\alpha,R)$.
  \item In order to prove that $\HAREACH$ satisfies the compositionality property,
        we lift Lemma~\ref{thm:zoo:track:congruence} to cover reachability as well.
        After that the compositionality property of $\HAREACH$ is verified analogously
        to the compositionality property of $\HATRACK$ (cf. Lemma~\ref{thm:zoo:track:compositional}).

        The lifting of Lemma~\ref{thm:zoo:track:congruence} is presented in Lemma~\ref{thm:zoo:reachability:congruence}.
        Similar to the proof of Lemma~\ref{thm:zoo:track:congruence:auxiliary},
        the proof of Lemma~\ref{thm:zoo:reachability:congruence} relies on an
        auxiliary property showing that
        \[ \REACH{x}{y}{\sh[\PS_1 / \rsh]} \quad\text{iff} \quad  \REACH{x}{y}{\sh\left[ \PS_1 / \SSIGMA{\CALLN{1}{}}{(B,\Lambda,S)} \right]} \]
        holds for all $x,y \in \VAR(\sh)$ and symbolic heaps $\sh$ containing a single predicate call $\PS_1$.
        This is formalized in Lemma~\ref{thm:zoo:reachability:congruence:auxiliary}.
\end{itemize}
%
Putting both together, we obtain a heap automaton $\HAREACH$ over $\SHCLASSFV{\alpha}$ accepting
$\RPROP(\alpha,R)$. 
Since the proofs required in this section are quite similar to the proofs in Section~\ref{app:zoo:track:property}, we refer to~\TECHNICALREPORT for the details.
\qed
%
\end{proof}
%

% $\PROJ{\T{v}_i}{j} \DEFEQ \begin{cases} \PROJ{\FV{0}{\rsh}}{j}, & \text{if} (i,j) \in S \\ z, & \text{otherwise} \end{cases}$.
%where $\T{v}_i = (\NIL,\PROJ{\FV{0}{\rsh}}{i_1},\ldots,\PROJ{\FV{0}{\rsh}}{i_n})$ such that $(i,j) \in S$ if and only if $j = i_k$ for some $1 \leq k \leq n$.
%
%
\begin{definition} \label{def:zoo:reachability-automaton}
 Let $\FV{0}{}$ be a tuple of variables with $\NOFV{} = \alpha \in \POSN$.
 %
 %
 Then $\HAREACH = (Q,\SHCLASSFV{\alpha},\Delta,F)$ is given by
 %accepting $\RPROP(\alpha,R)$ is given by:
%
  \begin{align*}
      Q ~\DEFEQ~ & Q_{\HAREACH} ~\times~ 2^{\FV{0}{} \times \FV{0}{}}, \qquad \quad F ~\DEFEQ~ Q_{\HATRACK} \times \{ R \} \\
      \Delta ~~:~~ & \MOVE{\HAREACH}{(q_0,S_0)}{\sh}{\T{p}},~ \T{p} = (q_1,S_1) \ldots (q_m,S_m) \\
    ~\text{iff}~ & \MOVE{\HATRACK}{q_0}{\varphi}{q_1 \ldots q_m} \\
                 & \text{and}~ \forall u,v \in \FV{0}{} ~.~
                     (u,v) \in S_0 \leftrightarrow \REACH{u^{\sh}}{v^{\sh}}{\SHRINK{\sh,\T{p}}}~,
  \end{align*}
  where
  \begin{align*}
     \SHRINK{\sh,\T{p}} ~\DEFEQ~ & \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{p}[1]}, \ldots, \PS_m / \SSIGMA{\CALLN{m}{}}{\T{p}[m]} \right].
  \end{align*}
%
Here, $m = \NOCALLS{\sh}$ stands for the number of predicate calls occurring in $\sh$ and $u^{\sh}$ denotes the free variable of $\sh$ corresponding to $u \in \FV{0}{}$.\footnote{formally if $u = \PROJ{\FV{0}{}}{i}$ then $u^{\sh} = \PROJ{\FV{0}{\sh}}{i}$}
%
Moreover, $q_i = (A_i,\Pi_i) \in Q_{\HATRACK}$ for each $0 \leq i \leq m$.
%
\end{definition}
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:reachability:language}
  $L(\HAREACH) = \RPROP(\alpha,R)$.
\end{lemma}
%
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:reachability:congruence:auxiliary}
 Let $\sh = \exists \BV{} . \SPATIAL{} \SEP \CALLN{1}{} : \PURE{} \in \SL{}{\SRDCLASSFV{\alpha}}$.
 %
 Moreover, let $\rsh \in \RSL{}{}$ with $\SIZE{\FV{0}{\rsh}} = \SIZE{\FV{1}{\sh}}$, $B = \{ y \in \FV{0}{} ~|~ y^{\rsh} \in \ALLOC{\rsh} \}$, $\Lambda = \{ x \sim y ~|~ x^{\rsh} \MSIM{\rsh} y^{\rsh} \}$, and
 %
 $S = \{ (x,y) \in \FV{0}{} \times \FV{0}{} ~|~ \REACH{x^{\rsh}}{y^{\rsh}}{\rsh} \}$.
 %
 Then, for each $x,y \in \VAR(\sh)$, we have
 %
 %
 \begin{align*}
    x \MSIM{\sh[\PS_1 / \rsh]} y \quad\text{iff}&\quad x \MSIM{\sh\left[ \PS_1 / \SSIGMA{\CALLN{1}{}}{(B,\Lambda,S)} \right]} y, \quad \text{and}~  \\
    x \in \ALLOC{\sh[\PS_1 / \rsh]} \quad\text{iff}&\quad x \in \ALLOC{\sh\left[ \PS_1 / \SSIGMA{\CALLN{1}{}}{(B,\Lambda,S)} \right]}, \quad \text{and}~  \\
    \REACH{x}{y}{\sh[\PS_1 / \rsh]} \quad\text{iff} &\quad  \REACH{x}{y}{\sh\left[ \PS_1 / \SSIGMA{\CALLN{1}{}}{(B,\Lambda,S)} \right]}~,
 \end{align*}
 %
 where $\rsha_{\PS_1\FV{1}{},(B,\Lambda,S)}$ has been defined at the beginning of this section.
 %
\end{lemma}
%
\begin{lemma} \label{thm:zoo:reachability:congruence}
 %
 Let $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m \geq 0$.
 %
 For each $1 \leq i \leq m$,
 let $\rsh_i \in \RSL{}{\SRDCLASSFV{\alpha}}$ with $\NOFV{\rsh_i} = \SIZE{\FV{i}{\sh}}$,
 $A_i = \{ y \in \FV{0} ~|~ y^{\rsh_i} \in \ALLOC{\rsh_i} \}$,
 $\PURE{}_i = \{ x \sim y ~|~ x^{\rsh_i} \MSIM{\rsh_i} y^{\rsh_i} \}$
 and $S_i  = \{ (x,y) \in \FV{0}{} \times \FV{0}{} ~|~ \REACH{x^{\rsh_i}}{y^{\rsh_i}}{\rsh_i} \}$.
 %
 Moreover, let
 %
 \begin{align*}
  \rsh ~\DEFEQ~ & \sh\left[\PS_1 / \rsh_1, \ldots, \PS_m / \rsh_m\right], \\
  \T{p} ~\DEFEQ~ & (A_1,\Pi_1,S_1) \ldots (A_m,\Pi_m,S_m), ~\text{and} \\
  \SHRINK{\sh,\T{p}} ~\DEFEQ~ & \sh\left[\PS_1 / \SSIGMA{\CALLN{1}{}}{\T{p}[1]},
                   \ldots,
                   \PS_m / \SSIGMA{\CALLN{m}{}}{\T{p}[m]}
                   \right].
 \end{align*}
 %
 Then, for each $x,y \in \VAR(\sh)$, we have
 \begin{align*}
   & x ~\MSIM{\rsh}~ y ~\text{iff}~  x ~\MSIM{\SHRINK{\sh,\T{p}}}~ y, \\ %\quad\text{and}\quad
   & x \in \ALLOC{\rsh} ~\text{iff}~ x \in \ALLOC{\SHRINK{\sh,\T{p}}}, \\
   %& \qquad  \qquad \qquad \qquad \quad \text{and}~ \quad
   & \REACH{x}{y}{\rsh} ~\text{iff}~ \REACH{x}{y}{\SHRINK{\sh,\T{p}}}. \qedhere
 \end{align*}
 %
\end{lemma}
%
%
\begin{proof}
  Analogous to the proof of Lemma~\ref{thm:zoo:track:congruence}
  except for the use of
  Lemma~\ref{thm:zoo:reachability:congruence:auxiliary} instead of
  Lemma~\ref{thm:zoo:track:congruence:auxiliary}.
  \qed
%
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Theorem~\ref{thm:zoo:reachability:complexity}} \label{app:zoo:reachability:complexity}
%
\begingroup
\def\thetheorem{\ref{thm:zoo:reachability:complexity}}
\begin{theorem}
  \DPROBLEM{SL-REACH} is \CCLASS{ExpTime}--complete and \CCLASS{coNP}--complete if the number of free variables is bounded.
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
   %
   Upper bounds are obtained as in the proof of Theorem~\ref{thm:zoo:establishment:complexity}.
   Thus,  we only show that the reduction provided in the paper proving the lower bounds is correct.
   %
   We first briefly recall how \COMPLEMENT{SL-RSAT} is reduced to \DPROBLEM{SL-REACH}.
   %
   Let $(\SRD,\PS)$ be an instance of \COMPLEMENT{SL-RSAT}.
   %
   Then an instance of \DPROBLEM{SL-REACH} is given by $(\SRD,\sh,\PROJ{\FV{0}{}}{1},\PROJ{\FV{0}{}}{2})$,  where
   %
   $ %\begin{align*}
    \sh ~\DEFEQ~ \exists \BV{} ~.~
        \PT{\PROJ{\FV{0}{}}{1}}{\NIL} \SEP \PS\BV{} ~:~ \{ \PROJ{\FV{0}{}}{2} \neq \NIL \}.
   $ %\end{align*}
   %
   Now,
   %
                       $\forall \rsh \in \CALLSEM{\sh}{\SRD} ~.~
                            \REACH{\PROJ{\FV{0}{}}{1}}{\PROJ{\FV{0}{}}{2}}{\rsh} 
    ~\Leftrightarrow~ 
                      \sh~\text{unsatisfiable}$. 
   A detailed proof of correctness is provided in~\TECHNICALREPORT.
   %
   Since $\sh$ is satisfiable if and only if $\PS$ is satisfiable by an analogous argument as in the proof of Lemma~\ref{thm:zoo:establishment:lower},
   it follows that
   $\REACH{\PROJ{\FV{0}{}}{1}}{\PROJ{\FV{0}{}}{2}}{\sh}$ holds for each $\rsh \in \CALLSEM{\sh}{\SRD}$
   if and only if $\PS$ is unsatisfiable.
   %
   \qed
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Lemma~\ref{thm:zoo:garbage:property}} \label{app:zoo:garbage:property}
%
\begingroup
\def\thelemma{\ref{thm:zoo:garbage:property}}
\begin{lemma}
 For each $\alpha \in \POSN$ the set $\GARBAGEPROP(\alpha)$, given by
 %
 \begin{align*}
   &\{ \rsh \in \RSL{}{\SRDCLASSFV{\alpha}} ~|~ \forall y \in \VAR(\rsh) ~.~ \exists x \in \FV{0}{\rsh} ~.~ 
   x \MEQ{\rsh} y ~\text{or}~ \REACH{x}{y}{\rsh} \}~,
 \end{align*}
 %
 of garbage-free symbolic heaps can be accepted by a heap automaton over $\SHCLASSFV{\alpha}$.
\end{lemma}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
%
We have to construct a heap automaton
$\HAGARBAGE$ over $\SHCLASSFV{\alpha}$ that satisfies the compositionality property
and accepts $\GARBAGEPROP(\alpha)$.
%
In order to highlight the necessary proof obligations, the actual construction of $\HAGARBAGE$
and its correctness proof are splitted into several definitions and lemmas that are
provided afterwards.
%

%
The construction of $\HAGARBAGE$ is similar to the construction of $\HAEST$
as presented in Theorem~\ref{thm:zoo:establishment}.
%
The main difference is that the reachability automaton $\HAREACH$,
formally introduced in Definition~\ref{def:zoo:reachability-automaton},
is used instead of the tracking automaton $\HATRACK$
and that the predicate $\CHECK$ is adapted.
A fully formal construction of $\HAGARBAGE$ is found in Definition~\ref{def:zoo:garbage:automaton}.
%
It then remains to show the correctness of our construction of $\HAGARBAGE$:
%
\begin{itemize}
  \item Lemma~\ref{thm:zoo:garbage:language} establishes that $\HAGARBAGE$ indeed accepts $\GARBAGEPROP(\alpha)$, i.e., $L(\HAGARBAGE) = \GARBAGEPROP(\alpha)$.
  \item To prove the compositionality property, we show that $\HAGARBAGE$ is an instance of a more general
        construction scheme whose compositionality property is shown in
        Lemma~\ref{thm:zoo:scheme:compositionality}.
        In order to apply Lemma~\ref{thm:zoo:scheme:compositionality}, we have to show that
        \begin{align*}
                          & \CHECK(\sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m], \EMPTYSEQ) = 1 \\
             ~\text{iff}~ & \CHECK(\sh,p_1 \ldots p_m) = 1 ~\text{and}~ \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1.
         \end{align*}
         This is verified in Lemma~\ref{thm:zoo:garbage:compositionality}.
         Then, by Lemma~\ref{thm:zoo:scheme:compositionality}, we already know that
         $\HAGARBAGE = \HASCHEME{\HAREACH}{\CHECK}{F}$ satisfies the compositionality property.
\end{itemize}
%
Putting both together, we obtain a heap automaton $\HAGARBAGE$ over $\SHCLASSFV{\alpha}$
that satisfies the compositionality property and accepts $\GARBAGEPROP(\alpha)$.
\qed
%
\end{proof}
%
\begin{definition} \label{def:zoo:garbage:automaton}
$\HAGARBAGE = (Q,\SHCLASSFV{\alpha},\Delta,F)$ is given by
%
\begin{align*}
   & Q ~\DEFEQ~ Q_{\HAREACH} \times \{0,1\} \qquad F ~\DEFEQ~ Q_{\HAREACH} \times \{1\} \\
   &  \Delta ~~:~~ \MOVE{\HAGARBAGE}{(p_0,q_0)}{\sh}{(p_1,q_1) \ldots (p_m,q_m)} \\
   & ~\text{iff}~ \MOVE{\HAREACH}{p_0}{\sh}{p_1\ldots p_m} \\
   & \qquad \text{and}~ q_0 = \min \{q_1,\ldots,q_m,\CHECK(\sh,p_1 \ldots p_m)\}~,
\end{align*}
%
where $\HAREACH$ is as in Definition~\ref{def:zoo:reachability-automaton}.
Furthermore, the predicate $\CHECK : \SHCLASSFV{\alpha} \times Q_{\HAREACH}^{*} \to \{0,1\}$
verifies that each variable of a symbolic heap $\sh$ is established in $\SHRINK{\sh,\T{p}}$,
where $\SHRINK{\sh,\T{p}}$ is the same as in the construction of $\HAREACH$.
%
Hence,
\begin{align*}
\CHECK(\sh,\T{p}) ~\DEFEQ~
 \begin{cases}
        1 &, ~\text{if}~ \forall y \in \VAR(\sh) \,.\, \exists x \in \FV{0}{\sh} ~.~ \\
          & \qquad        x \MEQ{\SHRINK{\sh,\T{p}}} y ~\text{or}~ \REACH{x}{y}{\SHRINK{\sh,\T{p}}} \\
        0 &, ~\text{otherwise}~,
 \end{cases}
\end{align*}
\end{definition}
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:garbage:language}
  %
  $L(\HAGARBAGE) = \GARBAGEPROP(\alpha)$.
  %
\end{lemma}
%
%
\begin{lemma} \label{thm:zoo:garbage:compositionality}
  Let  $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m$
  and $\rsh_1,\ldots,\rsh_m \in \RSL{}{\SRDCLASSFV{\alpha}}$. Then
  %
  \begin{align*}
                   & \CHECK(\sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m], \EMPTYSEQ) = 1 \\
      ~\text{iff}~ & \CHECK(\sh,\T{p}) 
                     ~\text{and}~ \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1. 
  \end{align*}
  %
\end{lemma}
%
The following technical observation, similar to Lemma~\ref{obs:zoo:establishment:equality-propagation}, is essential.
%
Intuitively, it states that a variable in one part of an unfolding is definitely reachable by a variable in a different part of an unfolding
only through a parameter (including $\NIL$) of one or more suitable predicate calls.
%
This is illustrated in Figure~\ref{fig:reach:propagation}.
%
\input{fig-reach-propagation}
%
\begin{lemma}[\TECHNICALREPORT] \label{obs:zoo:reachability:propagation}
 Let  $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m$,  $\rsh_1,\ldots,\rsh_m \in \RSL{}{\SRDCLASSFV{\alpha}}$ and
 $\rsh = \sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m]$.
 %
 Moreover, for $1 \leq i \leq m$, let $x \in \VAR(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}])$ and $y \in \VAR(\rsh) \setminus \VAR(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}])$.
 %
 Then $\REACH{x}{y}{\rsh}$ holds if and only if there exists $z \in \FV{i}{\sh}$ such that
 %
 \begin{itemize}
   \item $x \MEQ{\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}]} z$ and and $\REACH{z}{y}{\rsh}$, or
   \item $\REACH{x}{z}{\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}]}$ and $z \MEQ{\rsh} y$, or
   \item $\REACH{x}{z}{\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}]}$ and $\REACH{z}{y}{\rsh}$.
 \end{itemize}
 %
 Furthermore, the same holds for the converse direction, which means if 
 $y \in \VAR(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}])$ and $x \in \VAR(\rsh) \setminus \VAR(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}])$.
\end{lemma}
%
Note that this observation relies on the fact that the reachability relation $\REACH{}{}{\sh}$ is defined with respect to \emph{all} models of $\sh$, not just a single one. Otherwise, the observation is wrong for symbolic heaps that are not established.
%

%
\begin{proof}[of Lemma~\ref{thm:zoo:garbage:compositionality}]
%
Let $\rsh = \CHECK(\sh[\PS^{\sh}_1 / \rsh_1, \ldots, \PS^{\sh}_m / \rsh_m])$.
%
Then:
%
\begin{align*}
                    & \CHECK(\rsh,\EMPTYSEQ) = 1 \\
  ~\Leftrightarrow~ & \left[ \text{Definition of}~\CHECK,\SHRINK{\rsh,\EMPTYSEQ} = \rsh \right] \\
                    & \forall y \in \VAR(\rsh) ~.~ \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y ~\text{or}~ \REACH{x}{y}{\rsh} \\
  ~\Leftrightarrow~ & \left[
                        \VAR(\rsh) = \VAR(\sh) \cup
                        \bigcup_{1 \leq i \leq m} \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right])
                      \right] \\
                    & \forall y \in \VAR(\sh) . \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y ~\text{or}~ \REACH{x}{y}{\rsh} \\
                    & \quad \text{and}~ \forall 1 \leq i \leq m ~.~
                      \forall y \in \VAR\left(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right]\right) ~.~
                        \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y ~\text{or}~ \REACH{x}{y}{\rsh} \\
  ~\Leftrightarrow~ & \left[ y \in \VAR(\sh),
                             ~\text{Lemma}~\ref{thm:zoo:reachability:congruence} \right] \\
                    & \forall y \in \VAR(\sh) ~.~ \exists x \in \FV{0}{\sh} ~.~ x \MEQ{\SHRINK{\sh,\T{p}}} y 
                             ~\text{or}~ \REACH{x}{y}{\SHRINK{\sh,\T{p}}} \\
                    & \quad \text{and}~ \forall 1 \leq i \leq m ~.~
                      \forall y \in \VAR\left(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right]\right) ~.~ 
                      \exists x \in \FV{0}{\rsh} ~.~ x \MEQ{\rsh} y ~\text{or}~ \REACH{x}{y}{\rsh} \\
  ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{obs:zoo:establishment:equality-propagation},~\text{Lemma}~\ref{obs:zoo:reachability:propagation} \right] \\
                    & \forall y \in \VAR(\sh) ~.~ \exists x \in \FV{0}{\sh} ~.~ x \MEQ{\SHRINK{\sh,\T{p}}} y ~\text{or}~ \REACH{x}{y}{\SHRINK{\sh,\T{p}}} \\
                    & \quad \text{and}~ \forall 1 \leq i \leq m ~.~
                      \forall y \in \VAR\left(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right]\right) ~. \\
                    & \qquad  \exists x \in \FV{0}{\rsh} ~.~ \exists z \in \FV{i}{\sh}  ~.~
                      \left( x \MEQ{\rsh} z ~\text{or}~ \REACH{x}{z}{\rsh} \right)  \\
                    & \qquad \qquad ~\text{and}~
                      \left( \REACH{z}{y}{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]} ~\text{or}~
                      z \MEQ{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]} y \right)  \\
  ~\Leftrightarrow~ & \left[ \exists a \exists b \equiv \exists b \exists a,
                            ~x,y \in \VAR(\sh) \right] \\
                    & \forall y \in \VAR(\sh) . \exists x \in \FV{0}{\sh} ~.~ \REACH{x}{y}{\SHRINK{\sh,\T{p}}} \\
                    & \quad \text{and}~ \forall 1 \leq i \leq m ~.~
                      \forall y \in \VAR\left(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right]\right) ~. \\
                    & \qquad \exists z \in \FV{i}{\sh}  ~.~
                      \left( \REACH{z}{y}{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]}
                      ~\text{or}~ z \MEQ{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]} y \right)  \\
  ~\Leftrightarrow~ & \left[ \text{Definition of}~\CHECK \right] \\
                    & \CHECK(\sh,\T{p}) = 1 ~\text{and}~ \forall 1 \leq i \leq m ~.~
                      \CHECK(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}],\EMPTYSEQ) = 1 \\
  ~\Leftrightarrow~ & \left[ \CHECK(\rsh_i[\FV{0}{\rsh_i} / \FV{i}{\sh}],\EMPTYSEQ) = 1
                             ~\text{iff}~ \CHECK(\rsh_i,\EMPTYSEQ) = 1 \right] \\
                    & \CHECK(\sh,\T{p}) = 1 ~\text{and}~ \forall 1 \leq i \leq m ~.~
                      \CHECK(\rsh_i,\EMPTYSEQ) = 1. \qedhere
\end{align*}
%
\qed
\end{proof}
%

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Theorem~\ref{thm:zoo:garbage:complexity}} \label{app:zoo:garbage:complexity}
%
\begingroup
\def\thetheorem{\ref{thm:zoo:garbage:complexity}}
\begin{theorem}
  \DPROBLEM{SL-GF}
  is \CCLASS{ExpTime}--complete in general and $\CCLASS{coNP}$--complete if $\alpha$ is bounded.
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
   %
   Since upper bounds are obtained analogously to Theorem~\ref{thm:zoo:establishment:complexity},
   we only show that the reduction provided in the paper proving the lower bounds is correct.
   %
   We first briefly recall how \COMPLEMENT{SL-RSAT} is reduced to \DPROBLEM{SL-GF}.
   %
   Let $(\SRD,\PS)$ be an instance of \COMPLEMENT{SL-RSAT}.
   %
   Then a corresponding instance of \DPROBLEM{SL-GF} is given by
   $(\SRD,\sh)$, where $\FV{0}{\sh} = x$ and
   %
    $\sh ~\DEFEQ~ \exists \BV{} z' ~.~ \SEP \PS\BV{} ~:~ \{ x = \NIL, z' \neq \NIL \}$.
   %
   Now,
   %
   \begin{align*}
                         \CALLSEM{\sh}{\SRD} \subseteq \GARBAGEPROP(\alpha) 
      ~\Leftrightarrow~
                         \sh~\text{unsatisfiable}.
   \end{align*}
   %
   A detailed correctness proof is provided in~\TECHNICALREPORT.
   %
   Since $\sh$ is satisfiable if and only if $\PS$ is satisfiable by an analogous argument as in the proof of Lemma~\ref{thm:zoo:establishment:lower},
   it follows that $\CALLSEM{\sh}{\SRD} \subseteq \GARBAGEPROP(\alpha)$ holds if and only if $\PS$ is unsatisfiable.
   %
   \qed
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Lemma~\ref{thm:zoo:acyclicity:property}} \label{app:zoo:acyclicity:property}
%
\begingroup
\def\thelemma{\ref{thm:zoo:acyclicity:property}}
\begin{lemma}
  For each $\alpha \in \POSN$, the set
  \begin{align*}
          \CYCLEPROP(\alpha) ~\DEFEQ~ & \{ \rsh \in \RSHCLASSFV{\alpha} ~|~
               \NIL \MNEQ{\rsh} \NIL 
               ~\text{or}~ \forall x \in \VAR(\rsh) ~.~
              \text{not}~ \REACH{x}{x}{\rsh}  \}
          %\CYCLEPROP(\alpha) ~\DEFEQ~ & \{ \rsh \in \RSL{}{\SRDCLASSFV{\alpha}} ~|~ \forall x,y ~.~ x \MNEQ{\rsh} y \\
          %                            & \qquad \text{implies}~\text{not}~\REACH{x}{y}{\rsh}~\text{or}~\text{not}~\REACH{y}{x}{\rsh} \}
  \end{align*}
  of all weakly acyclic symbolic heaps can be accepted by a heap automaton over $\SHCLASSFV{\alpha}$.
\end{lemma}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
%
We have to construct a heap automaton
$\HACYCLE$ over $\SHCLASSFV{\alpha}$ that satisfies the compositionality property
and accepts $\CYCLEPROP(\alpha)$.
%
In order to highlight the necessary proof obligations, the actual construction of $\HACYCLE$
and its correctness proof are splitted into several definitions and lemmas that are
provided afterwards.
%

%
The construction of $\HACYCLE$ is similar to the construction of $\HAEST$
as presented in Theorem~\ref{thm:zoo:establishment}.
%
The main difference is that the reachability automaton $\HAREACH$,
formally introduced in Definition~\ref{def:zoo:reachability-automaton},
is used instead of the tracking automaton $\HATRACK$
and that the predicate $\CHECK$ is adapted.
A fully formal construction of $\HACYCLE$ is found in Definition~\ref{def:zoo:acyclicity:automaton}.
%
It then remains to show the correctness of our construction of $\HACYCLE$:
%
\begin{itemize}
  \item Lemma~\ref{thm:zoo:acyclicity:language} establishes that $L(\HACYCLE) = \CYCLEPROP(\alpha)$.
  \item To prove the compositionality property, we show that $\HACYCLE$ is an instance of a more general
        construction scheme whose compositionality property is shown in
        Lemma~\ref{thm:zoo:scheme:compositionality}.
        In order to apply Lemma~\ref{thm:zoo:scheme:compositionality}, we have to show that
        \begin{align*}
                          & \CHECK(\sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m], \EMPTYSEQ) = 1 \\
             ~\text{iff}~ & \CHECK(\sh,p_1 \ldots p_m) = 1 
                          ~\text{and}~ \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1.
         \end{align*}
         This is verified in Lemma~\ref{thm:zoo:acyclicity:compositionality}.
         Then, by Lemma~\ref{thm:zoo:scheme:compositionality}, we already know that
         $\HACYCLE = \HASCHEME{\HAREACH}{\CHECK}{F}$ satisfies the compositionality property.
\end{itemize}
%
%
Putting both together, we obtain a heap automaton $\HACYCLE$ over $\SHCLASSFV{\alpha}$
that satisfies the compositionality property and accepts $\CYCLEPROP(\alpha)$.
\qed
%
\end{proof}
%
\begin{definition} \label{def:zoo:acyclicity:automaton}
  $\HACYCLE = (Q,\SHCLASSFV{\alpha},\Delta,F)$ is given by
\begin{align*}
   & Q ~\DEFEQ~ Q_{\HAREACH} \times \{0,1\} \\
   & F ~\DEFEQ~ Q_{\HAREACH} \times \{1\} 
    ~\cup~ \{ (A,\Pi,S) \in Q_{\HAREACH} ~|~ \NIL \neq \NIL \in \Pi \} \times \{0\}  \\
   &  \Delta ~~:~~ \MOVE{\HACYCLE}{(p_0,q_0)}{\sh}{(p_1,q_1) \ldots (p_m,q_m)} \\
   & ~\text{iff}~ \MOVE{\HAREACH}{p_0}{\sh}{p_1\ldots p_m} 
   ~\text{and}~ q_0 = \min \{q_1,\ldots,q_m,\CHECK(\sh,p_1 \ldots p_m)\}~,
\end{align*}

%
where $\HAREACH$ is is as in Definition~\ref{def:zoo:reachability-automaton}.
Furthermore, the predicate $\CHECK : \SHCLASSFV{\alpha} \times Q_{\HAREACH}^{*} \to \{0,1\}$
verifies that each variable of a symbolic heap $\sh$ is not reachable from itself in $\SHRINK{\sh,\T{p}}$,
where $\SHRINK{\sh,\T{p}}$ is the same as in the construction of $\HAREACH$.
%
Hence,
%
\begin{align*}
\CHECK(\sh,\T{p}) ~\DEFEQ~
 \begin{cases}
        1 &, ~\text{if}~ \forall y \in \VAR(\sh) ~.~ \text{not}~\REACH{x}{x}{\SHRINK{\sh,\T{p}}} \\
        0 &, ~\text{otherwise}.
 \end{cases}
\end{align*}
\end{definition}
%
\begin{lemma}[\TECHNICALREPORT] \label{thm:zoo:acyclicity:language}
  %
  $L(\HACYCLE) = \CYCLEPROP(\alpha)$.
  %
\end{lemma}
%
%
\begin{lemma} \label{thm:zoo:acyclicity:compositionality}
  Let  $\sh \in \SL{}{\SRDCLASSFV{\alpha}}$ with $\NOCALLS{\sh} = m$
  and $\rsh_1,\ldots,\rsh_m \in \RSL{}{\SRDCLASSFV{\alpha}}$. Then
  %
  \begin{align*}
                   & \CHECK(\sh[\PS_1^{\sh} / \rsh_1, \ldots, \PS_m^{\sh} / \rsh_m], \EMPTYSEQ) = 1 \\
      ~\text{iff}~ & \CHECK(\sh,\T{p}) \\
                   & \text{and}~ \CHECK(\rsh_1,\EMPTYSEQ) = \ldots = \CHECK(\rsh_m,\EMPTYSEQ) = 1. \qedhere
  \end{align*}
  %
\end{lemma}
%
\begin{proof}
%
Let $\rsh = \CHECK(\sh[\PS^{\sh}_1 / \rsh_1, \ldots, \PS^{\sh}_m / \rsh_m])$.
%
Then
%
\begin{align*}
                   & \CHECK(\rsh,\EMPTYSEQ) = 1 \\
 ~\Leftrightarrow~ & \left[ \text{Definition of}~\CHECK, \rsh = \SHRINK{\rsh,\EMPTYSEQ} \right] \\
                   & \forall x \in \VAR(\rsh) ~.~ \text{not}~ \REACH{x}{x}{\rsh} \\
 ~\Leftrightarrow~ & \left[
                        \VAR(\rsh) = \VAR(\sh) \cup
                        \bigcup_{1 \leq i \leq m} \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right])
                      \right] \\
                   & \forall x \in \VAR(\sh) ~.~ \text{not}~ \REACH{x}{x}{\rsh} \\
                   & \text{and}~ \forall 1 \leq i \leq m ~.~
                         \forall x \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right])
                             ~.~ \text{not}~ \REACH{x}{x}{\rsh} \\
 ~\Leftrightarrow~ & \left[ \text{Lemma}~\ref{thm:zoo:reachability:congruence:auxiliary}  \right] \\
                   & \forall x \in \VAR(\sh) ~.~ \text{not}~ \REACH{x}{x}{\SHRINK{\sh,\T{p}}} \\
                   & \text{and}~ \forall 1 \leq i \leq m ~.~
                        \forall x \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right])
                             ~.~ \text{not}~ \REACH{x}{x}{\rsh}.
\end{align*}
%
Assume towards a contradiction that $\CHECK(\rsh_i,\EMPTYSEQ) = 0$ for some $1 \leq i \leq m$.
%
By definition and $\SHRINK{\rsh_i,\EMPTYSEQ} = \rsh_i$, this means that $\REACH{x}{x}{\rsh_i}$.
%
However, since $\rsh_i$ is contained in $\rsh$, this means that $\REACH{x}{x}{\rsh}$
and thus $\CHECK(\rsh,\EMPTYSEQ) = 0$.
%

%
Conversely, assume $\CHECK(\rsh,\EMPTYSEQ) = 0$, but $\CHECK(\sh,\T{p}) = 1$
and $\CHECK(\rsh_i,\EMPTYSEQ) = 1$ for each $1 \leq i \leq m$.
%
Thus,
%
\begin{align*}
                   & \forall x \in \VAR(\sh) ~.~ \text{not}~ \REACH{x}{x}{\SHRINK{\sh,\T{p}}} \tag{$\clubsuit$} \\
                   & \text{and}~ \forall 1 \leq i \leq m ~.~  \tag{$\spadesuit$}
                     \forall x \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh}  \right])
                         ~.~ \text{not}~ \REACH{x}{x}{\rsh_i}
\end{align*}
%
Then, there exists $x \in \VAR(\rsh)$ such that $\REACH{x}{x}{\rsh}$.
%
We proceed by case distinction:
%
\begin{enumerate}
  \item Case: $x \in \VAR(\sh)$.
        Then we immediately obtain a contradiction due to $(\clubsuit)$.
  %
  \item Case:
        $\REACH{x}{x}{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]}$ holds.
        Since
        $\REACH{x}{x}{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]}$
        holds if and only if
        $\REACH{x}{x}{\rsh_i}$ holds, we immediately obtain a contradiction due to $(\spadesuit)$.
  %
  \item Case:
        For some $1 \leq i \leq m$,
        $x \in \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right])$
        and
        $\REACH{x}{x}{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]}$
        does not hold.
        Then there exists
        $y \in \VAR(\rsh) \setminus \VAR(\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right])$
        such that one of the following two cases holds:
        \begin{enumerate}
            \item $x \MEQ{\rsh} y$ and $\REACH{y}{y}{\rsh}$.
                  Then, by Lemma~\ref{obs:zoo:establishment:equality-propagation},
                  there exists $z \in \FV{i}{\sh}$ such that
                  $x \MEQ{\rsh_i\left[ \FV{0}{\rsh_i} / \FV{i}{\sh} \right]} z$
                  and
                  $z \MEQ{\rsh} y$.
                  However, by construction of $\SHRINK{\sh,\T{p}}$, this means that $\REACH{z}{z}{\SHRINK{\sh,\T{p}}}$ holds, which
                  contradicts $(\clubsuit)$.
            \item $\REACH{x}{y}{\rsh}$ and $\REACH{y}{x}{\rsh}$.
                  Then, by Lemma~\ref{obs:zoo:reachability:propagation},
                  there exist $u,v \in \FV{i}{\sh}$ such that
                  $\REACH{u}{v}{\rsh}$ and $\REACH{v}{u}{\rsh}$.
                  However, by construction of $\SHRINK{\sh,\T{p}}$, this means that $\REACH{u}{u}{\SHRINK{\sh,\T{p}}}$ holds.
                  Thus $\CHECK(\sh,\T{p}) = 0$, which contradicts $(\clubsuit)$.
        \end{enumerate}
\end{enumerate}
%
Since each case leads to a contradiction, we conclude $\CHECK(\rsh,\T{p}) = 1$.
%
\qed
\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Proof of Theorem~\ref{thm:zoo:acyclicity:complexity}} \label{app:zoo:acyclicity:complexity}
%
\begingroup
\def\thetheorem{\ref{thm:zoo:acyclicity:complexity}}
\begin{theorem}
  \DPROBLEM{SL-AC}
  is \CCLASS{ExpTime}--complete in general and $\CCLASS{coNP}$--complete if $\alpha$ is bounded.
\end{theorem}
\addtocounter{theorem}{-1}
\endgroup
%
\begin{proof}
   %
   Upper bounds are obtained analogously to Theorem~\ref{thm:zoo:establishment:complexity}.
   Thus, we only show that the reduction provided in the paper proving the lower bounds is correct.
   %
   We first briefly recall how \COMPLEMENT{SL-RSAT} is reduced to \DPROBLEM{SL-AC}.
   %
   Let $(\SRD,\PS)$ be an instance of \COMPLEMENT{SL-RSAT}.
   %
   Then an instance of \DPROBLEM{SL-AC} is given by $(\SRD,\sh)$,
   where $\FV{0}{\sh} = x$ and
   $\sh = \exists \BV{} . \PT{x}{x} \SEP \PS\BV{}$.
   %
   Then
   %
   \begin{align*}
                        \CALLSEM{\sh}{\SRD} \subseteq \CYCLEPROP(\alpha) 
      ~\Leftrightarrow~ 
                        \sh~\text{unsatisfiable}.
   \end{align*}
   %
   A detailed correctness proof is provided in~\TECHNICALREPORT.
   %
   Now, by an analogous argument as in the proof of Theorem~\ref{thm:zoo:establishment:complexity},
   we obtain that $\sh$ is satisfiable iff $\PS$ is satisfiable.
   %
   Then $\CALLSEM{\sh}{\SRD} \subseteq \CYCLEPROP(\alpha)$ holds iff $\PS$ is unsatisfiable.
   %
   Hence, $\DPROBLEM{SL-AC}$ holds for $(\SRD,\sh)$ iff $\COMPLEMENT{SL-RSAT}$ holds for $(\SRD,\PS)$.
   %
   \qed
\end{proof}
%
%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> equivalence-classes.tex <==
\subsection{Systematic Construction of $\USET{\sh}{\SRD}{\CENTAIL{\alpha}}$}\label{sec:entailment:systematic}
%\paragraph{Systematic Construction of $\USET{\sh}{\SRD}{\CENTAIL{\alpha}}$}
Using heap automata to discharge entailments as presented in Theorem~\ref{thm:entailment:main}
requires the construction of suitable heap automata for each predicate symbol
of an SID.
% occurring in an SID.
%
We briefly present a systematic construction of such heap automata that is
similar to the well-known Myhill--Nerode Theorem for regular (tree) languages~\cite{comon2007tree,nerode1958linear}:
%
We partition the set of all reduced symbolic heaps into equivalence classes, where two formulas belong to the
same equivalence class if they can be extended in the same way to formulas entailing a predicate $\PS$ of interest.
%
%More formally,
%
\begin{definition} \label{def:subst-eq}
   %Let $\PS$ be a predicate symbol of an SID $\SRD$.
   Let $\PS \in \PRED(\SRD)$, $\SRD \in \SETSRD{}$.
   Then two symbolic heaps $\rsh,\rsha \in \RSL{}{\CENTAIL{\alpha}}$ with $\NOFV{\rsh} = \NOFV{\rsha} = \beta$
   are \emph{$\PS$--equivalent}, written $\rsh \EE{\PS} \rsha$,
   if for all $\sh \in \SL{}{}$ with exactly one predicate call $\PI$ of arity $\beta$,
   we have $\sh[\PI / \rsh] \ENTAIL{\emptyset} \PS\FV{0}{}$ iff
   $\sh[\PI / \rsha] \ENTAIL{\emptyset} \PS\FV{0}{}$.
\end{definition}
%
For example, all non-empty singly linked list segments
of the \texttt{sll} predicate from Section~\ref{sec:introduction} % Example~\ref{ex:srd}
with $\IFV{1}$ as head and $\IFV{2}$ as tail are $\texttt{sll}$--equivalent.
%
\begin{theorem}%[Myhill--Nerode~\cite{nerode1958linear}] 
   \label{thm:eq:myhill}
   Let $\PS$ be a predicate symbol of an SID $\SRD$.
   %
   Then there exists a heap automaton $\HASH{\PS}$ with
   $L(\HASH{\PS}) = \USET{\PS\FV{0}{}}{\SRD}{\CENTAIL{\alpha}}$ %\CALLSEM{\PS\FV{0}{}}{\SRD}$
   iff
   the number of equivalence classes of $\EE{\PS}$ is finite.
\end{theorem}
%
\begin{proof}
  Assume there are only finitely many equivalence classes of $\EE{\PS}$.
  Furthermore, let $\EC{\rsh}{\PS}$ denote the equivalence class containing formula $\rsh$.
  Then a heap automaton $\HASH{\PS} = (Q,\SHCENTAIL{\alpha},\Delta,F)$ accepting
  $\USET{\PS\FV{0}{}}{\SRD}{\CENTAIL{\alpha}}$
  is given by
  $Q = \{ \EC{\rsh}{\PS} ~|~ \rsh \in \RSL{}{\CENTAIL{\alpha}} \}$,
  $F = \{ \EC{\rsh}{\PS} ~|~ \rsh \in \RSL{}{\CENTAIL{\alpha}}, \rsh \ENTAIL{\SRD} \PS\FV{0}{} \}$
  and
  \begin{align*}
    \MOVE{\HASH{\PS}}{\EC{\sh[\CALLN{1}{} / \rsh_1, \CALLN{m}{} / \rsh_m]}{\PS}}{\sh}{\EC{\rsh_1}{\PS} \ldots \EC{\rsh_m}{\PS}}~,
  \end{align*}
  for each symbolic heap $\sh \in \SHCENTAIL{\alpha}$ with $\NOCALLS{\sh} = m$.
  %
  Then it is easy to verify that $\HA{A}$ satisfies the compositionality property
  and $L(\HASH{\PS}) = \USET{\PS\FV{0}{}}{\SRD}{\CENTAIL{\alpha}}$.
  %
  The converse direction is straightforward.
  %
  A full proof is found in Appendix~\ref{app:eq:myhill}.
  %
\end{proof}
%
Note that it suffices to represent each equivalence class by a single
reduced symbolic heap, e.g. the smallest one.
%
%Moreover, the equivalence classes themselves can be represented by predicates of an SID.
%
%
While the construction principle from above is generally applicable, it is, however,
often preferable to exploit other properties of the predicates of interest,
e.g., acyclicity (see Section~\ref{sec:zoo:acyclicity}), to reduce the number of equivalence classes.
%
A detailed example 
%of such a construction 
is provided in Section~\ref{sec:decidable-fragments}.
%
\subsection{Expressive Power}
%We conclude this section with a brief remark regarding the expressiveness of heap automata.
In general, a suitable heap automaton, as shown in Theorem~\ref{thm:eq:myhill},
can be constructed for any set of reduced symbolic heaps whose %underlying 
models
(interpreted as graphs) can be specified in monadic second-order logic~\cite{courcelle2012graph}.
%
This is a consequence of
the close relationship between established SIDs and context-free graph languages
that has been studied by Dodds et al.~\cite[Theorem
1]{dodds2008separation} %, Jansen et al.~\cite{jansen2014generating},
and Courcelle's work on recognizable graph languages~\cite[Theorems 4.34 and 5.68]{courcelle2012graph},
which are covered by heap automata due to Theorem~\ref{thm:eq:myhill}.
%
In particular, this means that each of the SL fragments studied in \cite{iosif2013tree,tatsuta2015separation,matheja2015treelike}
-- the most general decidable fragments known so far -- are within the scope of our approach.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fixed.tex <==
%
We conclude the technical part with an illustration of
the systematic construction of heap automata for entailment that we
introduced in the previous section: We determine the equivalence
classes $\EE{\mathtt{tll}}$, where the SID \texttt{tll} is defined as
in Example~\ref{ex:srd}, to obtain a heap automaton for the set of
well-determined reduced symbolic heaps that entail some tree with
linked leaves (TLL). Note that this SID is outside the scope of previous
decision procedures for entailment with (at most) exponential-time
complexity~\cite{berdine2004decidable,iosif2014entailment}.

For simplicity of presentation, we assume that %throughout this section that
all parameters of the \texttt{tll} predicate are different from $\NIL$
and consider only acyclic TLLs.\footnote{The only parameter that can
  actually be null is $\IFV{3}$, as the other two parameters are
  always equal to a variable that appears on the left-hand side of a
  points-to assertion. Likewise, $\IFV{3}$ is the only parameter that
  can introduce a cycle---it can be equal to $\IFV{1}$ or $\IFV{2}$.}
Recall that we can always check whether these conditions are satisfied
(see Sections~\ref{sec:zoo:track}, \ref{sec:zoo:acyclicity}); they are,
however, not essential for our construction to work.
%---in
%App.~\ref{app:tll-with-nil}, we show that it is also possible to
%remove the restrictions without an increase in asymptotic
%complexity.
%
Appendix~\ref{app:more-data-structures} illustrates the automaton
construction for singly-linked acyclic list segments.
%as introduced in
%the other two data structures of
%Example~\ref{ex:srd}.
%
Moreover, various kinds of trees are considered in Appendix~\ref{app:entailment:lower}.
%, singly-linked acyclic list segments and
%doubly-linked list segments.
%

%We follow the approach of defining each
%$\EE{\mathtt{tll}}$--equivalence class with an SID, as
%outlined below Theorem~\ref{thm:eq:myhill}.
We will represent each $\EE{\mathtt{tll}}$--equivalence class by an SID
whose unfoldings are exactly the reduced symbolic heaps contained in the respective class.
To this end, let \texttt{core} be a predicate specifying TLLs that lack the outgoing pointer of the right-most leaf:
%Formally,
\[
\begin{array}{l}
\PCDS{core} ~\SRDARROW~ \EMP : \{\IFV{1} = \IFV{2}\} \\
\PCDS{core} ~\SRDARROW~ \exists \ell\,r\,z ~.~ \PT{
  \IFV{1} }{ \ell\,r\,\NIL } \\ \qquad\qquad\quad \SEP ~ \PCDS{tll}{(\ell\,\IFV{2}\,z)} \SEP \PCDS{core}{(r\,z\,\IFV{3})}
\end{array}
\]
Here, the omitted pointer is reflected by the missing points-to assertion in the base case.
%Intuitively, the heaps defined by \texttt{core} are trees with linked
%leaves that lack the outgoing pointer of the right-most leaf, which is
%reflected in a difference in the base case.
%
In the following, let $\PERMS$ be the set of all permutations of
$\FV{0}{}$.
  \newcommand{\rhTfv}{\T{y}_{0}}
  \newcommand{\rhfv}{\PIFV} % Variables to use on the right-hand side
                            % of the rules
\newcommand{\tllclasses}{
  \begin{enumerate}
  \item $\ITLLC{1}\ ~\SRDARROW~ \PT{ \rhfv{1} }{
      \rhfv{2}\,\rhfv{3}\,\NIL }$
  \item $\ITLLC{2}\ ~\SRDARROW~ \PT{ \rhfv{1} }{ \NIL\,\NIL\,\rhfv{3}
    } ~:~ \{ \rhfv{1} = \rhfv{2} \}$
  \item $\ITLLC{3}\ ~\SRDARROW~ \PT{ \rhfv{1} }{ \NIL\,\NIL\,\rhfv{3}
    } ~:~ \{ \rhfv{2} = \rhfv{3} \}$
  \item $\ITLLC{4}\ ~\SRDARROW~ \PT{ \rhfv{1} }{ \NIL\,\NIL\,\rhfv{3}
    } ~:~ \PUREA{}$

  where $\PUREA{} \DEFEQ{} \{ \rhfv{1} \neq \rhfv{2}, \rhfv{2} \neq \rhfv{3} \}$

  \item $\ITLLC{5}\ ~\SRDARROW~
    \PCDS{core}{\rhTfv}$ %(Note: Subsumes empty.)
  \item $
      \ITLLC{6}\ ~\SRDARROW~ \exists \ell \, r \, z ~.~ \PT{
        \rhfv{1} }{ \ell\, r\, \NIL }$%\linebreak

      $\qquad\qquad ~\SEP\, \PCDS{tll}{(\ell\, \rhfv{2}\, z)} \SEP
      \PCDS{tll}{(r\, z\, \rhfv{3})}$

    %(Note: Must have first recursion step to separate this from $\ITLLC{2}$.)
  \item  $\ITLLC{7}\ ~\SRDARROW~ \exists u \, \ell \, r \, z ~.~ \PTS{\rhfv{2}}{u} \SEP \PT{
        \rhfv{1} }{ \ell\, r\, \NIL }$%\linebreak

     $\qquad\qquad ~\SEP\, \PCDS{tll}{(\ell\,u\,z)} \SEP
      \PCDS{core}{(r\, z\, \rhfv{3})}$

    %(Note: Must have first recursion step to separate this from $\ITLLC{2}$.)

  \item  $\ITLLC{8}\ ~\SRDARROW~ \exists u ~.~ \PT{\rhfv{2}}{(\NIL\,
      \NIL\, u)} \SEP \PCDS{tll}{(\rhfv{1}\, u\, \rhfv{3})}$
  % (Note: Subsumes the case with two link edges and nothing else.)
  \end{enumerate}
}
%
\begin{example} \label{ex:tll-classes} For each $\PERM \in \PERMS$,
  the relation $\EE{\mathtt{tll}}$ has 8 equivalence classes
  %of symbolic heaps
  that can be extended to entail an unfolding of
  \texttt{tll}:
  % Membership in these classes can be decided by checking
  % entailment against the following SIDs, where
  % $\PIFV{i} \DEFEQ \PERM(\IFV{i})$.

  \tllclasses{}
  We refer the reader to Figure~\ref{fig:fixed:tll} for an illustration of the unfoldings covered by each predicate. 
  Due to lack of space, this figure is found in the appendix.
  In addition, $\EE{\mathtt{tll}}$ has one equivalence class of
  symbolic heaps that cannot be extended to entail \texttt{tll}
  unfoldings, defined as the complement of the other classes:
  $\RSHCLASSFV{\alpha} \setminus \bigcup_{1 \leq i \leq 8, \PERM \in
    \PERMS} \ITLLC{i}$ \qedhere
\end{example}
%
For example, $\ITLLC{7}$ specifies all trees with linked leaves that
consist of more than one pointer, lack the successor of the rightmost
leaf, but have an additional element at the head of the list of linked
leaves. All such symbolic heaps can be extended to heaps that entail
an unfolding of $\PCDS{tll}{\FV{0}{}}$ in the same way; for
example by adding the missing pointer from the last leaf to its successor
and adding a new root node that points to the additional leaf at the head
of the list as well as to the root of the
$\ITLLC{7}$--unfolding. Formally, for the identity permutation
$\fid \in \PERMS$, let
\[
  \begin{array}{l}
\sh^{\fid} ~\DEFEQ{}~ \exists u \, v ~.~ \PT{\IFV{1}}{\IFV{2}\, u\,
    \NIL} \SEP \ \APP{P_7^{\fid}}{(u\,\IFV{2}\, v)} %\\\qquad\qquad
    \SEP \ \PT{v}{\NIL\,\NIL\, \IFV{3 }}.
  \end{array}
\]
Then $\sh^{\fid}\,\FV{0}{} \ENTAIL{} \PCDS{tll}{\FV{0}{}}$. Note that if we
change the predicate call from $P_7^{\fid}$ to $\ITLLC{7}$ for a
different $\PERM$, the parameters in the predicate call have to
be reordered in accordance with $\PERM$ to obtain a valid entailment
$\sh^{\PERM} \ENTAIL{} \PCDS{tll}{\FV{0}{}}$; hence different permutations
induce different equivalence classes.
%\footnote{The only
  % exception to this rule are the classes that do not completely define
  % the relationship between all parameters: Some of the classes defined
  % by $P_{2}$ and $P_{3}$ collapse, i.e.,
  % $\CALLSEM{P_i^{\PERM}\, \T{x}}{} = \CALLSEM{P_i^{\PERM'}\, \T{x}}{}$
  % for some $\PERM,\PERM' \in \PERMS$ and $i \in \{2,3\}$.}
A proof of Example~\ref{ex:tll-classes} is found
in Appendix~\ref{app:tll-classes}.
%
As there are six permutations of
$\FV{0}{}$, we conclude %that
\begin{corollary}\label{cor:tll-automaton}
  Let $\SRD$ be the SID defining \textnormal{\texttt{tll}} from
  Example~\ref{ex:srd}.  There is a heap automaton
  $\HA{A}_{\mathtt{tll}}$ with $8 \cdot 6 + 1 = 49$ states that
  accepts the set $\USET{\mathtt{tll}\,\T{x}}{\SRD}{\CENTAIL{3}}$.
  %of
  %reduced symbolic heaps that entail a \textnormal{\texttt{tll}} unfolding.
\end{corollary}

\begin{remark}
  One might be tempted to think that we have only moved the complexity
  into the transition relation and thus gained nothing:
  Instead of checking entailment w.r.t.~\texttt{tll}, we now have to
  verify entailments w.r.t.~several new SIDs.
  %We have
  %reduced entailment checking w.r.t.~\texttt{tll} to entailment
  %checking w.r.t.~several new SIDs.
  However, the states of our heap automaton coincide with
 % Note, however, that because the
 % states coincide with
  the $\EE{\texttt{tll}}$-equivalence classes.
  Thus, it always suffices to evaluate the transition relation w.r.t.~ to small \emph{canonical
   representations} of each equivalence class.
  %(cf.~Section~\ref{sec:entailment:systematic}).
  %
  Hence, instead of solving entailments of the
  % our heap automaton reduces large entailment problems of the
  form $P\, \T{x} \ENTAIL{} \mathtt{tll}\, \T{x}$ % to many small
  it suffices to consider entailments
 % instances of entailment problems
  $\rsh \ENTAIL{} \ITLLC{i}\, \T{x}$,
  where $\rsh$ is a \emph{reduced} symbolic heap.
  %Based on $\HA{A}_{\mathtt{tll}}$ we can thus decide the
  %entailment problem for symbolic heaps with \texttt{tll} predicates
  %in a compositional way.
  Moreover, since we assume well-determined symbolic heaps, each such
  $\rsh$ has a single tight model up to isomorphism.
  Then verifying $\rsh \ENTAIL{} \ITLLC{i}\, \T{x}$ boils down to the
  model-checking problem for fixed SIDs $\ITLLC{i}$. It follows by
  Remark~\ref{rem:model-checking} that
  $\Delta_{\HA{A}_{\mathtt{tll}}}$ is decidable in time
  $\BIGO{2^{\text{poly}(\SIZE{\SRD})}}$ (where $\SRD$ is the SID for
  $\mathtt{tll}$ from Example~\ref{ex:srd}).
  We thus apply
  Lemma~\ref{thm:entailment:exptime} to conclude that Algorithm~\ref{alg:entailment:decision-procedure}
  -- if fed with $\HA{A}_{\mathtt{tll}}$ -- is an \CCLASS{ExpTime} decision procedure for
  entailments containing \texttt{tll} predicates.
 % boils down to
 %    isomorphism checking of
 %    %$\sh[P_1/\rsh_{q_1}, \ldots, P_m/\rsh_{q_m}](\T{x})$
 %    $\rsh$ against those unfoldings of $\ITLLC{i}\,\T{x}$ that have
 %    the same number of points-to assertions.  For a small formula
 %    $\sh$ and small $\rsh$, the number of such unfoldings is
 %    small. For each unfolding, isomorphism can be checked
 %    efficiently.
\end{remark}

\begin{remark}
  Heap automata allow for easy integration of additional syntactic conditions
  in order to obtain more compact state spaces. % and thus boost performance.
  For instance, one observation is that many states of $\HA{A}_{\mathtt{tll}}$ collapse if
  reordering of parameters is restricted.

  Another approach is to fix the SID in advance and construct an
  automaton
  $\HA{A}^{\SRD} = (Q, \SL{\SRD}{\CENTAIL{\alpha}}, F, \Delta)$ that
  is only defined on symbolic heaps in
  $\SL{\SRD}{\CENTAIL{\alpha}}$. Depending on $\SRD$, there may be
  many $\EE{\PS}$--equivalence classes $\EC{\tau}{\PS}$ with
  $\EC{\tau}{\PS} \cap \SL{\SRD}{\CENTAIL{\alpha}} = \emptyset$.
  Dropping such classes can lead to significantly smaller
  automata---see App.~\ref{app:ha-size-fixed-srd} for an example. By
  restricting heap automata in this way, we obtain decision procedures
  for (established) symbolic heaps with fixed (as opposed to user-defined)
  SIDs, such as the original decidable symbolic heap
  fragment introduced by Berdine et al.~\cite{berdine2004decidable}.
\end{remark}


  %%% Local Variables:
  %%% mode: latex
  %%% TeX-master: "main"
  %%% End:


==> related-work.tex <==
Given the large body of literature on logics for specifying data structures, we concentrate on the work closely related to this paper.

\paragraph{Entailment Checking}

A lot of work has been invested on finding decision procedures for the entailment problem of symbolic heap fragments of separation logic~\cite{reynolds2002separation} with (fixed) recursive definitions.
The first work in this direction is due to Berdine et al.~\cite{berdine2004decidable}, where the entailment problem of a fragment with singly-linked lists only is shown to be decidable.
Most decidability results for restricted fragments with general inductive predicate definitions rely on a reduction to the satisfiability problem of monadic second-order logic over graphs~\cite{iosif2013tree, matheja2015treelike, tatsuta2015separation}.
However, this approach results in non-elementary decision procedures~\cite{meyer1975weak}.
To our best knowledge, no elementary complexity bounds are known for these general cases.
Antonopoulos et al.~\cite{antonopoulos2014foundations} showed that the entailment problem is undecidable in general and at least $\CCLASS{ExpTime}$--hard for the aforementioned restricted fragments.
Additionally, if heaps are always tree-shaped, Iosif et al.~\cite{iosif2014entailment} provide an $\CCLASS{ExpTime}$--complete decision procedure to check whether an entailment between two predicate calls holds.
This approach is based on tree automata, but does not cover entailments between general symbolic heaps over these restricted predicates.
Our results might help to extend their approach towards a decidable fully fledged fragment of symbolic heaps.

Moreover, Enea et al.\cite{enea2014entailment} develop a semi--decision procedure for a variety of fragments.
While their approach is based on compositional reasoning, it is, in contrast to our approach, incomplete and restricted to list--like predicates.

Other sound, but incomplete approaches have been proposed and successfully are applied by a variety of verification tools~\cite{berdine2011slayer,calcagno2011infer,chin2012automated, dudka2011predator, jacobs2011verifast, magill2008thor}.
In particular, Chin et al.~\cite{chin2012automated} used unfold/fold reasoning and Brotherston et al.~\cite{brotherston2011automated, brotherston2014cyclic} developed a cyclic proof system to discharge entailments.

\paragraph{Robustness Properties of SRDs}
Apart from the entailment problem, robustness properties of systems of recursive definitions are of practical interest.
For example, the satisfiability problem has been studied in~\cite{brotherston2014decision} to avoid wasting time on unrealistic scenarios during program analysis.
Furthermore, the model-checking problem is of interest in the context of run--time verification~\cite{brotherston2016model}.
Both problems have been shown to be $\CCLASS{ExpTime}$--complete by Brotherston et al~\cite{brotherston2014decision, brotherston2016model}.
Moreover, the establishment property turns out to be necessary for certain fragments studied by Iosif et al.~\cite{iosif2013tree, iosif2014entailment}.
Note that each of the aforementioned properties nicely fits into our framework of heap automata.
Other robustness properties, e.g. acyclicity and establishment turn out to be important in the context of termination analysis~\cite{zanardini2014inference} and to obtain decidable fragments~\cite{iosif2013tree, iosif2014entailment}, respectively.


\paragraph{Shape Analysis}
Our decision and refinement procedures are intended to be useful in the context of shape analysis of heap manipulating programs.
The first shape analysis of this kind is due to Sagiv et al.~\cite{sagiv1998solving}.
Corresponding analysis approaches based on separation logic have been developed subsequently~\cite{berdine2005symbolic, berdine2007shape, calcagno2009compositional, le2014shape}.
Furthermore, this kind of shape analysis has been extended to the concurrent setting by \cite{ohearn2007resources, brookes2007semantics} and studied in a thread-modular setting~\cite{gotsman2007thread}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

